RODEO: Robust Outlier Detection via Exposing Adaptive Out-of-Distribution Samples

In recent years, there have been significant improvements in various forms of image outlier detection. However, outlier detection performance under adversarial settings lags far behind that in standard settings. This is due to the lack of effective exposure to adversarial scenarios during training, especially on unseen outliers, leading to detection models failing to learn robust features. To bridge this gap, we introduce RODEO, a data-centric approach that generates effective outliers for robust outlier detection. More specifically, we show that incorporating outlier exposure (OE) and adversarial training can be an effective strategy for this purpose, as long as the exposed training outliers meet certain characteristics, including diversity, and both conceptual differentiability and analogy to the inlier samples. We leverage a text-to-image model to achieve this goal. We demonstrate both quantitatively and qualitatively that our adaptive OE method effectively generates ``diverse'' and ``near-distribution'' outliers, leveraging information from both text and image domains. Moreover, our experimental results show that utilizing our synthesized outliers significantly enhances the performance of the outlier detector, particularly in adversarial settings.

==> Diffusion.tex <==
 %\section{ Diffusion Models}
% \paragraph{OOD detection under adversarial attack:} In adversarial attacks on anomaly detection performance of neural networks with an additional exposure class, a basic PGD attack on cross-entropy loss, given by $x^{t+1} = x^t + \alpha \cdot \text{sgn}(\ell_{\theta}(x^t,y))$, proves inadequate, as perturbations between in-distribution classes do not impair OOD detection. Instead, an attack based on the anomaly score is employed, represented by $x^{t+1} = x^t + \alpha \cdot \text{sgn}(\ell_{\theta}(x^t,K+1) \cdot t)$ where $t$ is +1 for exposure samples and -1 for in-distribution samples. This approach aims to increase the final logit (anomaly score) for in-distribution samples and decrease it for exposure samples.





% Consider a data distribution $x_0 \sim q(x_0)$. A forward noising process generates a sequence of latents $x_1, \ldots, x_T$ by adding Gaussian noise with variance $\beta_t \in (0, 1)$ at each time step $t$:
% \begin{equation} \label{SDE_eq_1}
%     \centering
%     \begin{split}
% q(x_1, \ldots, x_T | x_0)  = \prod_{t=1}^T q(x_t | x_{t-1}) ,\ \ \ \ q(x_t | x_{t-1}) =\mathcal{N}(\sqrt{1 - \beta_t} x_{t-1}, \beta_t \mathbf{I})
%     \end{split}
% \end{equation}
% When $T$ is sufficiently large, the final latent $x_T$ closely resembles an isotropic Gaussian distribution. A notable characteristic of the forward noising process is that any step $x_t$ can be directly sampled from $x_0$, without  the need to create intermediate steps:
% \begin{equation} \label{SDE_eq_2}
%     \centering
%     \begin{split}
% q(x_t | x_0) \ = \mathcal{N}(\sqrt{\bar{\alpha}_t} x_0, (1 - \bar{\alpha}_t) \mathbf{I}), \ \ \ \
% x_t = \sqrt{\bar{\alpha}_t} x_0 + \sqrt{1 - \bar{\alpha}_t} \epsilon,
%     \end{split}
% \end{equation}


% Here, $\epsilon \sim \mathcal{N}(0, \mathbf{I}), \alpha_t=1-\beta_t$ and $\bar{\alpha}_t=\prod_{j=0}^t \alpha_j$. In order to obtain a new sample from the distribution $q(x_0)$, the Markovian process is reversed. Initiated with a Gaussian noise sample $x_T \sim \mathcal{N}(0, \mathbf{I})$, a reverse sequence is produced by sampling the posteriors $q(x_{t-1} | x_t)$, which are also Gaussian distributions \cite{feller2015theory,sohl2015deep}. In order to approximate this procedure, a neural network can be employed and trained as follows: $p_\theta(x_{t-1} | x_t) = \mathcal{N}(  \mu_\theta(x_t, t), \Sigma_\theta(x_t, t))$. This network takes the noisy image $x_t$ and the embedding at time step $t$ as input and learns to predict the mean $\mu_\theta(x_t, t)$ and the covariance $\Sigma_\theta(x_t, t)$.

% Hossein \textbf{Conditional Generation and Guidance }
%   Conditional generation \cite{kanizo2013palette,rombach2022high,zhang2023adding}, offering precise control over the content, is more crucial for practical applications. Various forms of conditions, such as labels, classifiers, texts, and images \cite{ho2022classifier,dhariwal2021diffusion,hong2022improving}, can be used to guide the generation process. \cite{dhariwal2021diffusion} modifies a class-conditional diffusion model by adjusting the mean based on the gradient of the log probability predicted by a classifier. The updated perturbed mean, $\hat{\mu}_\theta(x_t|y)$, is calculated as $\mu_\theta(x_t|y) + s \cdot \Sigma_\theta(x_t|y)\nabla_{x_t} \log p_\phi(y|x_t)$. Vision-language models, such as CLIP \cite{radford2021learning}, underpin successful text-conditioned diffusion models like DALL-E2 \cite{ramesh2022hierarchical} and GLIDE \cite{nichol2021glide}. These models leverage the guidance provided by noised CLIP models, employing the product of image and caption encodings ($enc_{img}(x_t).enc_{caption}(y)$) as a proxy for $log p(y|x_t)$ in guidance.

% The authors of GLIDE \cite{nichol2021glide} employed a CLIP \cite{radford2021learning} model in place of a classifier in classifier guidance. They modified the reverse-process mean by incorporating the gradient of the dot product of the image and caption encodings with respect to the image:  $\hat{\mu}_\theta(x_t|c) = \mu_\theta(x_t|c) + s \cdot \Sigma_\theta(x_t|c)\nabla_{x_t} (f(x_t) \cdot g(c))$, To acquire the accurate gradient in the reverse process, they trained CLIP on noisy images $x_t$.


% Image editing models have traditionally concentrated on tasks such as style transfer or converting between image domains. Given that  CLIP provides a score of how similar an image is to a caption, Many recent models among them have utilized CLIP embeddings for text-guided image editing. Among the numerous state-of-the-art text-to-image models, GLIDE works in pixel space. In contrast, many other techniques involve inverting or encoding images into a latent space, allowing for image manipulations by controlling latent vectors.



% \textbf{Conditional Generation and Guidance:} Unconditional generation allows for unconstrained exploration of a model's diverse sampling capabilities; however, conditional generation [refs], offering precise control over content, is more crucial for practical applications. Diffusion models excel in controllability and generate high-quality, diverse samples. Various forms of conditions, such as labels[refs], classifiers[refs], texts[refs], and images[refs], can be used to guide the generation process.

% Classifier Guidance [refs], using score function $\nabla log p(x_t|y) = \nabla log p(x_t) + s.\nabla log p(y|x_t)$, is one method for controlling the conditioning effect. Limited labels might restrict data distribution capture and generalization power. Additional semantic information, like textual descriptions and visual cues, can enhance data representation in generated samples. Vision-language models, such as CLIP, underpin successful text-conditioned diffusion models like DALL-E2[refs] and GLIDE[refs]. These models leverage the guidance provided by noised CLIP models, employing the product of image and caption encodings ($enc_{img}(x_t).enc_{caption}(y)$) as a proxy for $log p(y|x_t)$ in guidance.

% Dhariwal \& Nichol (2021) observed that the quality of samples from class-conditional diffusion models can often be improved using classifier guidance. This method involves perturbing a class-conditional diffusion model, which has a mean µθ(xt|y) and a variance Σθ(xt|y), by adding the gradient of the log probability log pϕ(y|xt) for a target class y as estimated by a classifier. The new perturbed mean, µˆθ(xt|y), is computed as µˆθ(xt|y) = µθ(xt|y) + s · Σθ(xt|y)∇xt log pϕ(y|xt). Dhariwal & Nichol (2021) found that the guidance scale, represented by the coefficient s, affects sample quality and diversity, with an increase in s improving sample quality while reducing diversity.
% \subsection{ GLIDE} 


% Various techniques involve inverting or encoding images into a latent space, enabling image manipulations by controlling latent vectors. On the other hand, GLIDE is one of the SOTA text-to-image model methods that operates at the pixel level.

% Among the numerous state-of-the-art text-to-image models, GLIDE operates in pixel space, while many others work in latent space. Despite the advantages of latent space models, such as reduced complexity and potential proficiency in semantic shifts, we choose GLIDE as our outlier generator, in line with our previously outlined approach. GLIDE’s ability to function in pixel space enables the generation of outliers with pixel-level flaws, an essential near-distribution shift for various applications, including industrial scenarios where pixel-level anomalies are prevalent. This type of shift might be difficult to achieve with latent space models, which is why GLIDE is our preferred choice.

% GLIDE operates in pixel space, while many others work in latent space. Despite the advantages of latent space models, such as reduced complexity and potential proficiency in semantic shifts, we choose GLIDE as our outlier generator, in line with our previously outlined approach. GLIDE's ability to function in pixel space enables the generation of outliers with pixel-level flaws, an essential near-distribution shift for various applications, including industrial scenarios where pixel-level anomalies are prevalent. This type of shift might be difficult to achieve with latent space models, which is why GLIDE is our preferred choice.



% %However, $q(x_{t-1} | x_t)$ remains unknown since it depends on the unidentified data distribution $q(x_0)$. To estimate this function, a deep neural network $p_\theta$ is employed to predict the mean and covariance of $x_{t-1}$, taking $x_t$ as input. Consequently, $x_{t-1}$ can be sampled from the normal distribution characterized by these parameters.     To obtain a new sample from the distribution $q(x_0)$, the Markovian process is reversed. Starting with a Gaussian noise sample $x_T \sim \mathcal{N}(0, \mathbf{I})$, a reverse sequence is created by sampling the posteriors $q(x_{t-1} | x_t)$, which are also Gaussian distributions \cite{feller2015theory,sohl2015deep}.     Nonetheless, $q(x_{t-1} | x_t)$ is not known since it depends on the unknown data distribution $q(x_0)$. To approximate this function, a deep neural network $p_\theta$ is used to predict the mean and covariance of $x_{t-1}$, with $x_t$ as input. Subsequently, $x_{t-1}$ can be sampled from the normal distribution defined by these parameters:

% $$
% p_\theta(x_{t-1} | x_t) = \mathcal{N}(\mu_\theta(x_t, t), \Sigma_\theta(x_t, t)).
% $$

% Instead of directly inferring $\mu_\theta(x_t, t)$, Ho et al. [24] suggest predicting the noise $\epsilon_\theta(x_t, t)$ that was added to $x_0$ to obtain $x_t$, according to Equation (2). Then, $\mu_\theta(x_t, t)$ can be derived using Bayes' theorem:

% $$
% \mu_\theta(x_t, t) = \frac{1}{\sqrt{\alpha_t}}\left(x_t - \frac{\beta_t}{\sqrt{1 - \bar{\alpha}t}} \epsilon\theta(x_t, t)\right)
% $$








% Forward Process: DDPMs, as mentioned in $[1]$ and $[2]$, gradually corrupt the training data with Gaussian noise. Let the data density be represented by $p(x_0)$, where the index 0 indicates the uncorrupted (original) data. Given an uncorrupted training sample $x_0 \sim p(x_0)$, the noisy versions $x_1, x_2, \ldots, x_T$ are generated using the following Markovian process:

% $$
% p(x_t | x_{t-1}) = \mathcal{N}(x_t; \sqrt{1 - \beta_t} \cdot x_{t-1}, \beta_t \cdot \mathbf{I}), \forall t \in {1, \ldots, T}
% $$

% Here, $T$ represents the total number of diffusion steps, and $\beta_1, \ldots, \beta_T \in [0, 1)$ are hyperparameters that define the variance schedule across the diffusion steps. $\mathbf{I}$ is the identity matrix with dimensions matching the input image $x_0$, while $\mathcal{N}(x; \mu, \sigma)$ denotes the normal distribution with mean $\mu$ and covariance $\sigma$ that yields $x$. A crucial characteristic of this recursive formulation is its ability to directly sample $x_t$ when $t$ is selected from a uniform distribution, i.e., $\forall t \sim \mathcal{U}({1, \ldots, T})$:

% $$
% p(x_t | x_0) = \mathcal{N}(x_t; \sqrt{\hat{\beta}_t} \cdot x_0, (1 - \hat{\beta}_t) \cdot \mathbf{I})
% $$


% \input{Figures/Third_Figure}



% DDPMs \cite{sohl2015deep,ho2020denoising} work to invert a parameterized Markovian image noise process, taking isotropic Gaussian noise samples as a starting point and transforming them into samples from a training distribution. This is achieved by progressively removing the noise via an iterative diffusion procedure.



%  Denoising Diffusion Probabilistic Models (DDPMs) \cite{sohl2015deep,ho2020denoising} establish a fixed Markov chain of latent distributions by incrementally introducing noise to input images and learning the inverse diffusion process to procure samples from input distributions. %These models offer advantages in generating content tailored to specific requirements, including enhanced control and adaptability [refs].
%  With samples $x_0 \sim q_0(x)$, DDPMs [refs] construct a T-step Markov chain of latent distributions $q_1(x)$,..., $q_T(x)$ through diffusion steps:
% $$
% q_t\left(x | x_{t-1}\right)=\mathcal{N}\left(x ; \sqrt{1-\beta_t} \cdot x_{t-1}, \beta_t \cdot \mathbf{I}\right), \ \ \ \forall t \in{1, \ldots, T}
% $$
% through learning reverse diffusion steps, one can sample the noise prior $q_T(x)$ and successively denoise the image until a sample is obtained from distribution $q_0(x)$. 


% Diffusion Models are a class of generative models that define a (usually fixed) Markov chain of diffusion processes that gradually add noise to input images and then learn the reverse of diffusion process in order to obtain samples of input distribution starting from the noise or easy to sample prior distributions.

% given samples $x_0 \sim q_0(x)$, denoising diffusion probabilistic models (DDPMs) define a T step markov chain of latent distributions $q_1(x)$, ..., $q_T(x)$ by adding noise to previous step samples in progressive diffusion steps:
% $$
% q_t\left(x | x_{t-1}\right)=\mathcal{N}\left(x ; \sqrt{1-\beta_t} \cdot x_{t-1}, \beta_t \cdot \mathbf{I}\right), \ \ \ \ \forall t \in\{1, \ldots, T\}
% $$
% with noises in each step ($\beta_t$) being small enough but total noise of $q_t(x|x_0)$ which is 1-$\prod_{i=1}^T (1-\beta_i)$ being large enough, the distribution of $x_t$ is approximately an isotropic standard gaussian distribution $\mathcal{N}(0, \mathbf{I})$  and also posterior distributions $q_{t-1}(x|x_t)$ are approximated by isotropic gaussians. by learning reverse diffusion steps one can sample from the noise prior $q_T(x)$ and then denoise the image step by step by sampling from posteriors until a sample is obtained from distribution $q_0(x)$.

% By direct calulation of $q_t(x|x_0)$ based on noise variables and subsituting in Bayes rule we can formulate posteriors in the $ q_{t-1}(x|x_t) \propto \mathcal{N}(\mu_q(x_t, x_0) , \Sigma(t) ) $ form. there are different derivations of variational lower-bound on log q$_0(x)$ or its surrogates which results in different ways of learning posteriors including training a network $ \hat{x_{\theta}}(x_t, t) $ to predict the original natural image $x_0$ from an arbitrary noised version $x_t$ [refs], a network $ \hat{\epsilon_{\theta}}(x_t, t) $ that learns to predict the source noise $\epsilon_0 \sim \mathcal{N}(0, \mathbf{I})$ that determines $x_t$ from $x_0$ [refs] or a network $s_{\theta}(x_t, t)$ that learns to predict the score function $\nabla_{x_t} log q_t(x)$ for any arbitrary noise level t [refs].

% \textbf{Conditional Generation and Guidance:} Unconditional generation allows for unconstrained exploration of a model's diverse sampling capabilities; however, conditional generation [refs], offering precise control over content, is more crucial for practical applications. Diffusion models excel in controllability and generate high-quality, diverse samples. Various forms of conditions, such as labels[refs], classifiers[refs], texts[refs], and images[refs], can be used to guide the generation process.

% Classifier Guidance [refs], using score function $\nabla log p(x_t|y) = \nabla log p(x_t) + s.\nabla log p(y|x_t)$, is one method for controlling the conditioning effect. Limited labels might restrict data distribution capture and generalization power. Additional semantic information, like textual descriptions and visual cues, can enhance data representation in generated samples. Vision-language models, such as CLIP, underpin successful text-conditioned diffusion models like DALL-E2[refs] and GLIDE[refs]. These models leverage the guidance provided by noised CLIP models, employing the product of image and caption encodings ($enc_{img}(x_t).enc_{caption}(y)$) as a proxy for $log p(y|x_t)$ in guidance.


% %While unconditional generation can be valuable in empirical studies as it allows for unconstrained exploration of the model's potential to generate diverse samples, conditional generation is more crucial for practical applications as it provides precise control over the generated content based on specific conditions or intentions.Diffusion models are particularly strong in terms of their controllability, and they can generate samples with high quality and diversity. Various forms of conditions are commonly employed to direct the generation process of diffusion models, including but not limited to labels, classifiers, texts, and images.

% % A diffusion model that is trained conditionally with label guidance could possibly devalue the provided conditioning information. another way of conditional generation with more control on conditioning effect is guidance. with classifier guidance the score of an unconditional diffusion model is learned as previously derived, alongside a classifier that takes in arbitrary noisy $x_t \sim q_t(x)$ and attempts to predict conditional information y. The score function learned under Classifier Guidance is:
% % $$
% % \nabla log p(x_t|y) = \nabla log p(x_t) + s.\nabla log p(y|x_t)
% % $$

% % To avoid the need for a separate classifier trained on noisy images, Considering that $ p(y|x_t) \propto \frac{p(x_t|y)}{p(x_t)} $ we can achieve classifier-free guidance with following score function:
% % $$
% % \nabla log p(x_t|y) = \nabla log p(x_t) + s.(\nabla log p(x_t|y) - \nabla log p(x_t) )
% % $$
% % $$
% % = (1-s).\nabla log p(x_t) + s.\nabla log p(x_t|y)
% % $$

% % Using labels to guide diffusion models can produce desirable samples, but limited labels may restrict the model's ability to capture the full data distribution and limit its generalization power. Incorporating additional semantic information, such as textual descriptions and visual cues, to condition diffusion models can capture nuanced aspects of the data distribution and improve the representation of complex semantics in generated samples, according to recent advances in applications of diffusion models.

% %  Vision-language models have attracted a lot of attention recently due to the number of potential applications. CLIP as scalable approach
% % for learning joint representations between text and images is main component of some succesful text-conditioned diffusion models like [DALL-E2 and GLIDE]. in CLIP-guided diffusion models the $enc_{img}(x_t).enc_{caption}(y)$ obatained from noised CLIP models is used as a proxy for $log p(y|x_t)$ in guidance.


% %Outlier exposure can help redefine the open set boundaries of the in-distribution and out-of-distribution classes by providing the detector with a more diverse set of OOD examples during training.  This can improve the detector's ability to distinguish between in-distribution and out-of-distribution examples, and to become more robust to new, unseen examples. the choice of distribution of exposures and the way that detector incorporates information of exposures are design choices that affect the abilities of detector in test time facing with OOD samples.

% %Exposures could be a general random dataset but also could be collected or generated task dependant. in task dependant exposures diversity and distance of exposures from in distribution is important to better define boundaries of distributions for detector. in classification based detectors models are trained with uniform label on exposure samples to be less confident on OOD samples or treat exposures as a seperate OOD class in training for learning better discrimination of ID and OOD samples.



==> Figures/HeatMap.tex <==
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=1\linewidth]{Images/fig-heatmap.pdf}
    \caption{The results demonstrate that when the targeted dataset and the exposed dataset have a smaller distance (as shown on the diagonal), the robustness results are better.}
    \label{fig:Comparison_Plot}
  \end{center}
\end{figure}


==> Figures/Theory.tex <==
\begin{figure}[h]
  \begin{center}
    \includegraphics[width=1\linewidth]{Images/fig-theory.pdf}
 %    \caption{Illustration of an insightful example in a one-dimensional feature space, where the outlier 
 % exposure distribution is a subset of the true outliers. The set of feasible thresholds that separate the training data perfectly (green, which is normal, and orange, which is the outlier exposure set) are gray colored. $r$ represents the amount of shift in exposed outliers with respect to the actual anomaly distribution. The subset of feasible values that lead to a perfect test AUROC are bold grays.
 % \\
 %  \textbf{Left}: The standard training and testing scenario. Perfect thresholds constitute a significant proportion of feasible values, even when the outlier exposure are located far from normal samples. 
 % \\
 % \textbf{Middle}: Using adversarial training, the set of feasible thresholds  reduces significantly due to the nature of maximum margin of adversarial training. This in turn reduces the set of perfect thresholds. A large deviation of outlier exposure samples from the actual anomaly distribution lead to a small set of perfect thresholds relative to the set of feasible thresholds. 
 % \\
 %  \textbf{Right}: In the case of adversarial testing, the overlap between the set of feasible and perfect thresholds shrinks to a single point $a$. This shows that the near-distribution property of the exposed outliers is more critical in the adversarial setting as it shrinks the relative size of the set of perfect solutions with respect to the feasible ones. }
     \caption{Effect of the outlier exposure distribution in a one-dimensional feature space in the adversarial and standard setups. Gray regions indicate feasible thresholds for separating the classes in the training data, where green represents the normal class and orange represents the outlier exposure. The parameter \(r\) measures the shift in exposed outliers relative to the actual anomalies, and bold grays indicate thresholds yielding perfect test AUROC values. \textbf{Left:} Standard training scenario with many perfect thresholds, even with distant outlier exposure. \textbf{Middle:} Adversarial training narrows the set of perfect thresholds by reducing the feasible options. \textbf{Right:} During adversarial testing, the set of perfect thresholds contracts to a single point \(a\), highlighting the criticality of near-distribution exposure in adversarial setups.}

    \label{fig:Comparison_Plot}
  \end{center}
\end{figure}


==> Tables/Background_and_Related_Works.tex <==
\section{Background and Related work}

% \paragraph{ND, OSR and OOD detection} \ In OSR, a model is trained on $K$ classes from an $N$-class training dataset. During testing, the model encounters $N$ distinct classes, where $N-K$ of these classes were not present during the training phase. ND is a type of open-set recognition that is considered an extreme case, specifically when $k$ is equal to 1. OOD detection shares similarities with OSR; however, the key distinction is that the open-set and closed-set classes originate from two separate datasets.\cite{yang2021generalized,mirzaei2022fake}




%In OSR, one typically deals with $M$ concepts (or classes) as the closed set, and $N-$ other  concepts as the open set. In this setting, concepts in the open set  usually constitute semantic categories of the same dataset that are not seen in the closed set. ND is a type of open-set recognition that is considered an extreme case, specifically when $M$ is equal to 1. 

%All of these categories consider two disjoint sets called the 'closed' (or 'normal') set and the 'open' (or 'anomalous') set. During the training phase, the model does not have access to the open set. However, during the testing phase, the model is presented with both the closed and open sets, and it must be able to discriminate between them. 


%Despite the fact that out-of-distribution detection, open-set recognition, and anomaly detection have similarities in their underlying concepts, most studies have focused on these areas independently. However, there has been an increased interest in approaching these topics from a more comprehensive perspective. OOD detection shares similarities with OSR; however, the key distinction is that the open-set and closed-set classes originate from two separate datasets.


%


%In OSR, one typically deals with $M$ concepts (or classes) as the closed set, and $N$ other  concepts as the open set. In this setting, concepts in the open set  usually constitute semantic categories of the same dataset that are not seen in the closed set. ND is a type of open-set recognition that is considered an extreme case, specifically when $M$ is equal to 1. 

%OOD detection is similar to OSR with the difference that the concepts in the open set are typically assumed to come from categories that are not peers of the ones in the closed set. It has to be noted that unlike ND, the closed set class labels are provided during training, and the model is expected to classify the input data into these classes as well as identifying closed vs. open sets at the inference time. Having access to the class labels often makes OSR and OOD detection an easier task than ND.
%When performing OOD detection, two different datasets are employed - the closed set and the open set. The absence of data labels as an additional information source during training separates ND from OSR and OOD techniques, which possess this capability. This attribute makes ND a more challenging undertaking. 
 \paragraph{Baselines}
Several methods have been proposed in ND, with a goal of learning the distribution of normal samples through self-supervised approaches. Ruff's approach entails learning the distribution's features using an autoencoder, whereas CSI applies a contrastive loss for distribution learning. Moreover, some other works aim to leverage the knowledge from pre-trained models. Furthermore, some other works have pursued ND in an adversarial setting, APAE suggests enhancing adversarial robustness through the utilization of approximate projection and feature weighting. PrincipaLS propose Principal Latent Space as a defense strategy to perform adversarially robust ND, OCSDF aims to
achieve robustness in OCC by learning a signed distance function to the boundary of the support of any distribution, which can be interpreted as a normality score. OSAD method augments the model architecture with dual-attentive denoising layers, and integrates the adversarial training loss with an auto-encoder loss. The auto-encoder loss is designed to reconstruct the original image from its adversarial counterpart.some other works  incorporate OE to enhance their performance in both clean and adversarial OOD detection evaluation tasks \cite{kong2021opengan,liznerski2022exposing,mirzaei2022fake}. The most direct approach to utilizing outliers involves incorporating them into the training set, with labels uniformly selected from the label space of typical samples. In an effort to improve the adversarial robustness of detection models, some methods have attempted to make OE more adaptive. For example, ATD \cite{azizmalayeri2022your} employs a generator to craft fake features instead of images. Another approach, ALOE \cite{chen2021atom}, mines low anomaly score data from an auxiliary  OOD dataset for training, thereby enhancing the robustness of OOD detection.
 
% \cite{hendrycks2018deep} introduced the  OE technique for OOD detection tasks, which is utilizing auxiliary random images known to be anomalous. Many top-performing OOD detection methods incorporate OE to enhance their performance in both classic and adversarial OOD detection evaluation tasks \cite{kong2021opengan,liznerski2022exposing,mirzaei2022fake}. The most direct approach to utilizing outliers involves incorporating them into the training set, with labels uniformly selected from the label space of typical samples. In an effort to improve the adversarial robustness of OOD detection, some methods have attempted to make OE more adaptive. For example, ATD \cite{azizmalayeri2022your} employs a generator to craft fake features instead of images. Another approach, ALOE \cite{chen2021atom}, mines low anomaly score data from an auxiliary  OOD dataset for training, thereby enhancing the robustness of OOD detection.


% This strategy can enhance the performance of certain anomaly detection methods, such as Maximum Softmax Probability (MSP) [ref]. Alternatively, outliers can be treated as a distinct class during training, which allows the logits of this new class in an arbitrary classifier to serve as an anomaly score.

\paragraph{Adversarial attacks} For input $x$ with an associated ground-truth label $y$, an adversarial example $x^*$ is generated by adding slight noise to $x$, maximizing the predictor model loss $\ell(x^*; y)$ in the process. To ensure that the image's semantics remain unchanged, the $l_p$ norm of the adversarial noise should not exceed a predetermined value $\epsilon$, specifically, $\left\|x-x^*\right\|_p \leq \epsilon$. The Projected Gradient Descent (PGD) \cite{madry2017towards} method is regarded as a standard and effective attack technique that functions by iteratively maximizing the loss function, utilizing a step size $\alpha$ in the direction of the gradient sign of $\ell(x^*; y)$ with respect to $x$:$\quad   x_0^*=x, \quad x_{t+1}^*=x_t^*+\alpha . \operatorname{sign}\left(\nabla_x \ell\left(x_t^*, y\right)\right),$ where the noise is to be projected onto the $\ell_{\infty}$-ball  with a radius of $\epsilon$ during each step.





==> Tables/Diffusion.tex <==
 %\section{ Diffusion Models}
% \paragraph{OOD detection under adversarial attack:} In adversarial attacks on anomaly detection performance of neural networks with an additional exposure class, a basic PGD attack on cross-entropy loss, given by $x^{t+1} = x^t + \alpha \cdot \text{sgn}(\ell_{\theta}(x^t,y))$, proves inadequate, as perturbations between in-distribution classes do not impair OOD detection. Instead, an attack based on the anomaly score is employed, represented by $x^{t+1} = x^t + \alpha \cdot \text{sgn}(\ell_{\theta}(x^t,K+1) \cdot t)$ where $t$ is +1 for exposure samples and -1 for in-distribution samples. This approach aims to increase the final logit (anomaly score) for in-distribution samples and decrease it for exposure samples.

\textbf{Denoising Diffusion Probabilistic Models (DDPMs)} 
DDPMs \cite{sohl2015deep,ho2020denoising} are trained to reverse a parameterized Markovian image noise process. Beginning with isotropic Gaussian noise samples, they iteratively convert these samples into ones from a training distribution while steadily eliminating noise through a diffusion process. The process can be divided into two main steps: the forward diffusion process and the reverse denoising process. Recent studies have demonstrated that DDPMs can generate high-quality images. \cite{dhariwal2021diffusion,avrahami2022blended,croitoru2023diffusion}



% Consider a data distribution $x_0 \sim q(x_0)$. A forward noising process generates a sequence of latents $x_1, \ldots, x_T$ by adding Gaussian noise with variance $\beta_t \in (0, 1)$ at each time step $t$:
% \begin{equation} \label{SDE_eq_1}
%     \centering
%     \begin{split}
% q(x_1, \ldots, x_T | x_0)  = \prod_{t=1}^T q(x_t | x_{t-1}) ,\ \ \ \ q(x_t | x_{t-1}) =\mathcal{N}(\sqrt{1 - \beta_t} x_{t-1}, \beta_t \mathbf{I})
%     \end{split}
% \end{equation}
% When $T$ is sufficiently large, the final latent $x_T$ closely resembles an isotropic Gaussian distribution. A notable characteristic of the forward noising process is that any step $x_t$ can be directly sampled from $x_0$, without  the need to create intermediate steps:
% \begin{equation} \label{SDE_eq_2}
%     \centering
%     \begin{split}
% q(x_t | x_0) \ = \mathcal{N}(\sqrt{\bar{\alpha}_t} x_0, (1 - \bar{\alpha}_t) \mathbf{I}), \ \ \ \
% x_t = \sqrt{\bar{\alpha}_t} x_0 + \sqrt{1 - \bar{\alpha}_t} \epsilon,
%     \end{split}
% \end{equation}


% Here, $\epsilon \sim \mathcal{N}(0, \mathbf{I}), \alpha_t=1-\beta_t$ and $\bar{\alpha}_t=\prod_{j=0}^t \alpha_j$. In order to obtain a new sample from the distribution $q(x_0)$, the Markovian process is reversed. Initiated with a Gaussian noise sample $x_T \sim \mathcal{N}(0, \mathbf{I})$, a reverse sequence is produced by sampling the posteriors $q(x_{t-1} | x_t)$, which are also Gaussian distributions \cite{feller2015theory,sohl2015deep}. In order to approximate this procedure, a neural network can be employed and trained as follows: $p_\theta(x_{t-1} | x_t) = \mathcal{N}(  \mu_\theta(x_t, t), \Sigma_\theta(x_t, t))$. This network takes the noisy image $x_t$ and the embedding at time step $t$ as input and learns to predict the mean $\mu_\theta(x_t, t)$ and the covariance $\Sigma_\theta(x_t, t)$.

\textbf{ Conditional Generation and Guidance }
  Conditional generation \cite{kanizo2013palette,rombach2022high,zhang2023adding}, offering precise control over the content, is more crucial for practical applications. Various forms of conditions, such as labels, classifiers, texts, and images \cite{ho2022classifier,dhariwal2021diffusion,hong2022improving}, can be used to guide the generation process. \cite{dhariwal2021diffusion} modifies a class-conditional diffusion model by adjusting the mean based on the gradient of the log probability predicted by a classifier. The updated perturbed mean, $\hat{\mu}_\theta(x_t|y)$, is calculated as $\mu_\theta(x_t|y) + s \cdot \Sigma_\theta(x_t|y)\nabla_{x_t} \log p_\phi(y|x_t)$. Vision-language models, such as CLIP \cite{radford2021learning}, underpin successful text-conditioned diffusion models like DALL-E2 \cite{ramesh2022hierarchical} and GLIDE \cite{nichol2021glide}. These models leverage the guidance provided by noised CLIP models, employing the product of image and caption encodings ($enc_{img}(x_t).enc_{caption}(y)$) as a proxy for $log p(y|x_t)$ in guidance.

% The authors of GLIDE \cite{nichol2021glide} employed a CLIP \cite{radford2021learning} model in place of a classifier in classifier guidance. They modified the reverse-process mean by incorporating the gradient of the dot product of the image and caption encodings with respect to the image:  $\hat{\mu}_\theta(x_t|c) = \mu_\theta(x_t|c) + s \cdot \Sigma_\theta(x_t|c)\nabla_{x_t} (f(x_t) \cdot g(c))$, To acquire the accurate gradient in the reverse process, they trained CLIP on noisy images $x_t$.


% Image editing models have traditionally concentrated on tasks such as style transfer or converting between image domains. Given that  CLIP provides a score of how similar an image is to a caption, Many recent models among them have utilized CLIP embeddings for text-guided image editing. Among the numerous state-of-the-art text-to-image models, GLIDE works in pixel space. In contrast, many other techniques involve inverting or encoding images into a latent space, allowing for image manipulations by controlling latent vectors.



% \textbf{Conditional Generation and Guidance:} Unconditional generation allows for unconstrained exploration of a model's diverse sampling capabilities; however, conditional generation [refs], offering precise control over content, is more crucial for practical applications. Diffusion models excel in controllability and generate high-quality, diverse samples. Various forms of conditions, such as labels[refs], classifiers[refs], texts[refs], and images[refs], can be used to guide the generation process.

% Classifier Guidance [refs], using score function $\nabla log p(x_t|y) = \nabla log p(x_t) + s.\nabla log p(y|x_t)$, is one method for controlling the conditioning effect. Limited labels might restrict data distribution capture and generalization power. Additional semantic information, like textual descriptions and visual cues, can enhance data representation in generated samples. Vision-language models, such as CLIP, underpin successful text-conditioned diffusion models like DALL-E2[refs] and GLIDE[refs]. These models leverage the guidance provided by noised CLIP models, employing the product of image and caption encodings ($enc_{img}(x_t).enc_{caption}(y)$) as a proxy for $log p(y|x_t)$ in guidance.

% Dhariwal \& Nichol (2021) observed that the quality of samples from class-conditional diffusion models can often be improved using classifier guidance. This method involves perturbing a class-conditional diffusion model, which has a mean µθ(xt|y) and a variance Σθ(xt|y), by adding the gradient of the log probability log pϕ(y|xt) for a target class y as estimated by a classifier. The new perturbed mean, µˆθ(xt|y), is computed as µˆθ(xt|y) = µθ(xt|y) + s · Σθ(xt|y)∇xt log pϕ(y|xt). Dhariwal & Nichol (2021) found that the guidance scale, represented by the coefficient s, affects sample quality and diversity, with an increase in s improving sample quality while reducing diversity.
% \subsection{ GLIDE} 


% Various techniques involve inverting or encoding images into a latent space, enabling image manipulations by controlling latent vectors. On the other hand, GLIDE is one of the SOTA text-to-image model methods that operates at the pixel level.

% Among the numerous state-of-the-art text-to-image models, GLIDE operates in pixel space, while many others work in latent space. Despite the advantages of latent space models, such as reduced complexity and potential proficiency in semantic shifts, we choose GLIDE as our outlier generator, in line with our previously outlined approach. GLIDE’s ability to function in pixel space enables the generation of outliers with pixel-level flaws, an essential near-distribution shift for various applications, including industrial scenarios where pixel-level anomalies are prevalent. This type of shift might be difficult to achieve with latent space models, which is why GLIDE is our preferred choice.

% GLIDE operates in pixel space, while many others work in latent space. Despite the advantages of latent space models, such as reduced complexity and potential proficiency in semantic shifts, we choose GLIDE as our outlier generator, in line with our previously outlined approach. GLIDE's ability to function in pixel space enables the generation of outliers with pixel-level flaws, an essential near-distribution shift for various applications, including industrial scenarios where pixel-level anomalies are prevalent. This type of shift might be difficult to achieve with latent space models, which is why GLIDE is our preferred choice.



% %However, $q(x_{t-1} | x_t)$ remains unknown since it depends on the unidentified data distribution $q(x_0)$. To estimate this function, a deep neural network $p_\theta$ is employed to predict the mean and covariance of $x_{t-1}$, taking $x_t$ as input. Consequently, $x_{t-1}$ can be sampled from the normal distribution characterized by these parameters.     To obtain a new sample from the distribution $q(x_0)$, the Markovian process is reversed. Starting with a Gaussian noise sample $x_T \sim \mathcal{N}(0, \mathbf{I})$, a reverse sequence is created by sampling the posteriors $q(x_{t-1} | x_t)$, which are also Gaussian distributions \cite{feller2015theory,sohl2015deep}.     Nonetheless, $q(x_{t-1} | x_t)$ is not known since it depends on the unknown data distribution $q(x_0)$. To approximate this function, a deep neural network $p_\theta$ is used to predict the mean and covariance of $x_{t-1}$, with $x_t$ as input. Subsequently, $x_{t-1}$ can be sampled from the normal distribution defined by these parameters:

% $$
% p_\theta(x_{t-1} | x_t) = \mathcal{N}(\mu_\theta(x_t, t), \Sigma_\theta(x_t, t)).
% $$

% Instead of directly inferring $\mu_\theta(x_t, t)$, Ho et al. [24] suggest predicting the noise $\epsilon_\theta(x_t, t)$ that was added to $x_0$ to obtain $x_t$, according to Equation (2). Then, $\mu_\theta(x_t, t)$ can be derived using Bayes' theorem:

% $$
% \mu_\theta(x_t, t) = \frac{1}{\sqrt{\alpha_t}}\left(x_t - \frac{\beta_t}{\sqrt{1 - \bar{\alpha}t}} \epsilon\theta(x_t, t)\right)
% $$








% Forward Process: DDPMs, as mentioned in $[1]$ and $[2]$, gradually corrupt the training data with Gaussian noise. Let the data density be represented by $p(x_0)$, where the index 0 indicates the uncorrupted (original) data. Given an uncorrupted training sample $x_0 \sim p(x_0)$, the noisy versions $x_1, x_2, \ldots, x_T$ are generated using the following Markovian process:

% $$
% p(x_t | x_{t-1}) = \mathcal{N}(x_t; \sqrt{1 - \beta_t} \cdot x_{t-1}, \beta_t \cdot \mathbf{I}), \forall t \in {1, \ldots, T}
% $$

% Here, $T$ represents the total number of diffusion steps, and $\beta_1, \ldots, \beta_T \in [0, 1)$ are hyperparameters that define the variance schedule across the diffusion steps. $\mathbf{I}$ is the identity matrix with dimensions matching the input image $x_0$, while $\mathcal{N}(x; \mu, \sigma)$ denotes the normal distribution with mean $\mu$ and covariance $\sigma$ that yields $x$. A crucial characteristic of this recursive formulation is its ability to directly sample $x_t$ when $t$ is selected from a uniform distribution, i.e., $\forall t \sim \mathcal{U}({1, \ldots, T})$:

% $$
% p(x_t | x_0) = \mathcal{N}(x_t; \sqrt{\hat{\beta}_t} \cdot x_0, (1 - \hat{\beta}_t) \cdot \mathbf{I})
% $$


% \input{Figures/Third_Figure}



% DDPMs \cite{sohl2015deep,ho2020denoising} work to invert a parameterized Markovian image noise process, taking isotropic Gaussian noise samples as a starting point and transforming them into samples from a training distribution. This is achieved by progressively removing the noise via an iterative diffusion procedure.



%  Denoising Diffusion Probabilistic Models (DDPMs) \cite{sohl2015deep,ho2020denoising} establish a fixed Markov chain of latent distributions by incrementally introducing noise to input images and learning the inverse diffusion process to procure samples from input distributions. %These models offer advantages in generating content tailored to specific requirements, including enhanced control and adaptability [refs].
%  With samples $x_0 \sim q_0(x)$, DDPMs [refs] construct a T-step Markov chain of latent distributions $q_1(x)$,..., $q_T(x)$ through diffusion steps:
% $$
% q_t\left(x | x_{t-1}\right)=\mathcal{N}\left(x ; \sqrt{1-\beta_t} \cdot x_{t-1}, \beta_t \cdot \mathbf{I}\right), \ \ \ \forall t \in{1, \ldots, T}
% $$
% through learning reverse diffusion steps, one can sample the noise prior $q_T(x)$ and successively denoise the image until a sample is obtained from distribution $q_0(x)$. 


% Diffusion Models are a class of generative models that define a (usually fixed) Markov chain of diffusion processes that gradually add noise to input images and then learn the reverse of diffusion process in order to obtain samples of input distribution starting from the noise or easy to sample prior distributions.

% given samples $x_0 \sim q_0(x)$, denoising diffusion probabilistic models (DDPMs) define a T step markov chain of latent distributions $q_1(x)$, ..., $q_T(x)$ by adding noise to previous step samples in progressive diffusion steps:
% $$
% q_t\left(x | x_{t-1}\right)=\mathcal{N}\left(x ; \sqrt{1-\beta_t} \cdot x_{t-1}, \beta_t \cdot \mathbf{I}\right), \ \ \ \ \forall t \in\{1, \ldots, T\}
% $$
% with noises in each step ($\beta_t$) being small enough but total noise of $q_t(x|x_0)$ which is 1-$\prod_{i=1}^T (1-\beta_i)$ being large enough, the distribution of $x_t$ is approximately an isotropic standard gaussian distribution $\mathcal{N}(0, \mathbf{I})$  and also posterior distributions $q_{t-1}(x|x_t)$ are approximated by isotropic gaussians. by learning reverse diffusion steps one can sample from the noise prior $q_T(x)$ and then denoise the image step by step by sampling from posteriors until a sample is obtained from distribution $q_0(x)$.

% By direct calulation of $q_t(x|x_0)$ based on noise variables and subsituting in Bayes rule we can formulate posteriors in the $ q_{t-1}(x|x_t) \propto \mathcal{N}(\mu_q(x_t, x_0) , \Sigma(t) ) $ form. there are different derivations of variational lower-bound on log q$_0(x)$ or its surrogates which results in different ways of learning posteriors including training a network $ \hat{x_{\theta}}(x_t, t) $ to predict the original natural image $x_0$ from an arbitrary noised version $x_t$ [refs], a network $ \hat{\epsilon_{\theta}}(x_t, t) $ that learns to predict the source noise $\epsilon_0 \sim \mathcal{N}(0, \mathbf{I})$ that determines $x_t$ from $x_0$ [refs] or a network $s_{\theta}(x_t, t)$ that learns to predict the score function $\nabla_{x_t} log q_t(x)$ for any arbitrary noise level t [refs].

% \textbf{Conditional Generation and Guidance:} Unconditional generation allows for unconstrained exploration of a model's diverse sampling capabilities; however, conditional generation [refs], offering precise control over content, is more crucial for practical applications. Diffusion models excel in controllability and generate high-quality, diverse samples. Various forms of conditions, such as labels[refs], classifiers[refs], texts[refs], and images[refs], can be used to guide the generation process.

% Classifier Guidance [refs], using score function $\nabla log p(x_t|y) = \nabla log p(x_t) + s.\nabla log p(y|x_t)$, is one method for controlling the conditioning effect. Limited labels might restrict data distribution capture and generalization power. Additional semantic information, like textual descriptions and visual cues, can enhance data representation in generated samples. Vision-language models, such as CLIP, underpin successful text-conditioned diffusion models like DALL-E2[refs] and GLIDE[refs]. These models leverage the guidance provided by noised CLIP models, employing the product of image and caption encodings ($enc_{img}(x_t).enc_{caption}(y)$) as a proxy for $log p(y|x_t)$ in guidance.


% %While unconditional generation can be valuable in empirical studies as it allows for unconstrained exploration of the model's potential to generate diverse samples, conditional generation is more crucial for practical applications as it provides precise control over the generated content based on specific conditions or intentions.Diffusion models are particularly strong in terms of their controllability, and they can generate samples with high quality and diversity. Various forms of conditions are commonly employed to direct the generation process of diffusion models, including but not limited to labels, classifiers, texts, and images.

% % A diffusion model that is trained conditionally with label guidance could possibly devalue the provided conditioning information. another way of conditional generation with more control on conditioning effect is guidance. with classifier guidance the score of an unconditional diffusion model is learned as previously derived, alongside a classifier that takes in arbitrary noisy $x_t \sim q_t(x)$ and attempts to predict conditional information y. The score function learned under Classifier Guidance is:
% % $$
% % \nabla log p(x_t|y) = \nabla log p(x_t) + s.\nabla log p(y|x_t)
% % $$

% % To avoid the need for a separate classifier trained on noisy images, Considering that $ p(y|x_t) \propto \frac{p(x_t|y)}{p(x_t)} $ we can achieve classifier-free guidance with following score function:
% % $$
% % \nabla log p(x_t|y) = \nabla log p(x_t) + s.(\nabla log p(x_t|y) - \nabla log p(x_t) )
% % $$
% % $$
% % = (1-s).\nabla log p(x_t) + s.\nabla log p(x_t|y)
% % $$

% % Using labels to guide diffusion models can produce desirable samples, but limited labels may restrict the model's ability to capture the full data distribution and limit its generalization power. Incorporating additional semantic information, such as textual descriptions and visual cues, to condition diffusion models can capture nuanced aspects of the data distribution and improve the representation of complex semantics in generated samples, according to recent advances in applications of diffusion models.

% %  Vision-language models have attracted a lot of attention recently due to the number of potential applications. CLIP as scalable approach
% % for learning joint representations between text and images is main component of some succesful text-conditioned diffusion models like [DALL-E2 and GLIDE]. in CLIP-guided diffusion models the $enc_{img}(x_t).enc_{caption}(y)$ obatained from noised CLIP models is used as a proxy for $log p(y|x_t)$ in guidance.


% %Outlier exposure can help redefine the open set boundaries of the in-distribution and out-of-distribution classes by providing the detector with a more diverse set of OOD examples during training.  This can improve the detector's ability to distinguish between in-distribution and out-of-distribution examples, and to become more robust to new, unseen examples. the choice of distribution of exposures and the way that detector incorporates information of exposures are design choices that affect the abilities of detector in test time facing with OOD samples.

% %Exposures could be a general random dataset but also could be collected or generated task dependant. in task dependant exposures diversity and distance of exposures from in distribution is important to better define boundaries of distributions for detector. in classification based detectors models are trained with uniform label on exposure samples to be less confident on OOD samples or treat exposures as a seperate OOD class in training for learning better discrimination of ID and OOD samples.



==> Tables/Introduction.tex <==

A widespread assumption in model development in machine learning is that the test data is drawn from the same distribution as the training data, known as the closed-set assumption. However, during inference, the model may encounter a wide variety of anomalous data that deviates significantly from the training distribution \cite{drummond2006open}. This phenomenon creates issues in safety-critical applications, which require detection and distinct treatment of anomalous data \cite{nguyen2015deep}. Several techniques have been developed for this purpose under various setups, which include novelty detection (ND), Out-of-Distribution (OOD) detection, and Open-Set Recognition (OSR) \cite{perera2021one,geng2020recent,yang2021generalized}. We seek to provide a robust and unified solution for these problems under adversarial attacks at inference time. Robustness to adversarial attacks is a key requirement in real-world model development. Adversarial attacks are the imperceptible input perturbations that are designed to cause the model to make incorrect predictions \cite{szegedy2013intriguing,goodfellow2014explaining,akhtar2018threat}. It is well known that the standard training makes the models vulnerable to such attacks in the classification problem \cite{madry2017towards,wong2020fast,zhang2019theoretically}, and in particular in the OOD detection \cite{chen2021atom,fort2022adversarial}.  This issue is more significant in OOD detection as it violates the main premise of such methods, which was to guard the model against unknown concepts in safety-critical applications \cite{chen2020robust}. OOD detection methods have not been successful in achieving ideal robust detection rates despite attempts to make them adversarially robust \cite{azizmalayeri2022your,lo2022adversarially,chen2020robust,shao2020open,shao2022open,bethune2023robust,goodge2021robustness,chen2021atom}. 
 
\input{Figures/First_Figure}
 


Adversarial training, which is the augmentation of training samples with adversarial perturbations, is among the best practices in making models robust. However, it is less effective in OOD detection as the anomalous patterns are not known during training, so one cannot train the model with adversarial perturbations associated with anomalies. For this reason, recent robust OOD detection methods use the outlier exposure (OE) technique \cite{hendrycks2018deep} in combination with adversarial training to tackle this issue \cite{azizmalayeri2022your,chen2020robust,chen2021atom}. In OE, traditionally, outlier samples are typically obtained from fixed datasets and are leveraged during training. It is clear that these samples should be semantically different from the normal training set to avoid misleading the detection.


Our experiments demonstrate that the performance of the OE technique, specifically in adversarial settings, is highly sensitive to the distance between the OE and the normal training set distribution. As shown in the figure\ref{fig:Comparison_Plot}, when ALOE \cite{chen2020robust} and ATD \cite{azizmalayeri2022your} use Tiny ImageNet \cite{imagenet} as an OE dataset for CIFAR10 \cite{krizhevsky2009learning} as the normal dataset, the results are significantly better compared to when we replace Tiny ImageNet with MNIST \cite{lecun-mnisthandwrittendigit-2010} as the OE for CIFAR-10. This suggests that an OE dataset closer to the normal dataset's distribution is significantly more beneficial than a distant one. This observation aligns with \cite{xing2022artificially}, which suggests that incorporating data near the decision boundary leads to a more adversarially robust model. Simultaneously, numerous studies \cite{schmidt2018adversarially,stutz2019disentangling} have demonstrated that adversarial training demands a greater level of sample complexity relative to the clean settings. Thus, several pioneering efforts have been made to enrich data diversity, either by integrating more data \cite{hendrycks2019usingx,zhai2019adversarially,najafi2019robustness,alayrac2019labels,carmon2019unlabeled,wang2019improving} or utilizing augmentation techniques \cite{wang2023better,rebuffi2021fixing,gowal2021improving,rade2021reducing,pang2022robustness,sehwag2021robust}, to enhance adversarial robustness. This observation prompts us to put forth the following proposition: {\it The set of outliers in OE methods need to be ``diverse'', ``near-distribution'', and conceptually differentiable from the normal samples, for the adversarial training to be effective in robust OOD detection.}

By the near-distribution outliers, we mean such data possess semantically and stylistically related characteristics to that of the normal set. If the outliers are not near-distribution, the classification boundary would be misplaced in the input space, causing a distribution shift on the adversarial perturbations of the outlier samples compared to those of the real anomalies. We have conducted numerous extensive ablation studies \ref{Ablation_Section} and provided theoretical insights \ref{Theory} to offer evidence for these claims. Driven by these insights, we propose an adaptive OE, a data generation technique that conditions the generation on the information from the distribution of the normal set. 

While some previous works \cite{azizmalayeri2022your,chen2021atom,mirzaei2022fake,kong2021opengan} have proposed conditional generation techniques to create more adaptable outliers compared to traditional methods (which used a fixed dataset for OE), they failed to achieve satisfactory results. This is because they only considered information in the image domain for conditioning. In contrast, we leveraged all available information in the normal set, including both images and text. Our ablation study demonstrated that excluding any of this information results in decreased performance.

 In our proposed method, we employ a pre-trained diffusion model \cite{nichol2021glide} to generate diverse and high-quality near-distribution OOD samples. To be more precise, assuming we have label(s) for a normal dataset (e.g., "Dog"), we use a simple text encoder model to extract words that are semantically similar to the normal labels but are distinct from them (e.g., "Wolf"). Using these near-OOD words, we guide the generative model to generate near-OOD data, conditioned on normal images. Our key idea here is that crafting outliers is often more manageable through simultaneous language and image processing. The empirical results from the ND setup on various tiny, medical, and industrial datasets, as well as the generalization of the method to OOD detection and OSR setups, demonstrate that our method, RODEO, significantly improves the mean area under the receiver operating characteristics (AUROC) under various adversarial attacks.


 
Our key results and contributions are:

\begin{itemize}
    \item We propose a novel method, adversarial training with adaptive outlier exposure, that allows for the efficient integration of auxiliary outlier data, resulting in robust OOD detection, ND, and OSR. Our method has achieved state-of-the-art performance by increasing the AUROC up to 50\%.
 
    \item 
 We extensively evaluate RODEO in various OOD detection environments, encompassing common benchmarks and adversarial tasks. Our testing involves one-class and multi-class settings. Significantly, we are the first to demonstrate all these settings under a single framework in the field of robust OOD detection.






% In OE, outlier samples that are typically obtained from other datasets are leveraged during training. OThis observation prompts us to put forth the following proposition:  {\it The set of outliers in OE methods need to be ``diverse'', ``near-distribution'', and conceptually differentiable from the normal samples, for the adversarial training to be effective in robust OOD detection.}

% The need for diverse outlier samples is often associated with the increased sample complexity in adversarial training. \cite{schmidt2018adversarially}. 
 
%  \item  Furthermore, our work involves an exploration of robust pretraining for the task of robust OOD detection. Notably, we have demonstrated for the first time that pre-trained adversarially robust neural networks on the ImageNet dataset can be leveraged to improve the results.
 %    \item
 % We provide theoretical insights on why outlier mining with high boundary scores benefits sample efficiency.


 % Motivated by this, we suggest an ad aptive OE technique utilizing guided diffusion models as a substitute for the prevalent random sampling method in the literature. We assume that the title(s) of the normal class(es) are known during training. Such titles are modified slightly through exploring the semantically rich embedding space generated by the Word2Vec model \cite{mikolov2013efficient}                                 to identify negative adjectives of a class, such as ``broken'' for the ``screw'' class, or word replacements such as ``nail'' for the ``screw'' class. The modified title is then given as a prompt to a pre-trained text-to-image generative model that is conditioned on a normal image to generate outliers for OE. Finally, a classifier is adversarially trained to distinguish generated outliers from the normal samples.

% The key idea here is that crafting outliers is often more manageable through the language, compared to directly making edits in the image space. Note that the latter may not necessarily turn a normal image into an anomalous one, while the former is better suited for this purpose. In addition, by searching for the words with the closest meaning to the normal titles, and also conditioning on the normal image, the generated outlier would be near-distribution. Leveraging pre-trained text-to-image generative models also helps in making diverse samples.The empirical results of ND setup on various tiny, medical, and industrial datasets, and also the generalization of the method to OOD detection and OSR setups, show that our method, RODEO, makes a huge improvement in the adversarial AUC under various attacks. 



% %Anomaly detection (AD) refers to the problem of determining if a test data sample is anomalous compared to a corpus of normal data. The application of deep neural networks is becoming more common in real-world settings that involve AD, such as medical diagnosis, industrial defect detection, and autonomous driving. Unfortunately, models are capable of producing unreliable confidence values for test samples that are not part of the training set.

 

% %All of these categories consider two disjoint sets called the 'closed' (or 'normal') set and the 'open' (or 'anomalous') set. During the training phase, the model does not have access to the open set. However, during the testing phase, the model is presented with both the closed and open sets, and it must be able to discriminate between them. Despite the fact that out-of-distribution detection, open-set recognition, and anomaly detection have similarities in their underlying concepts, most studies have focused on these areas independently. However, there has been an increased interest in approaching these topics from a more comprehensive perspective.


% %


% %In OSR, one typically deals with $M$ concepts (or classes) as the closed set, and $N$ other  concepts as the open set. In this setting, concepts in the open set  usually constitute semantic categories of the same dataset that are not seen in the closed set. ND is a type of open-set recognition that is considered an extreme case, specifically when $M$ is equal to 1. 

% %OOD detection is similar to OSR with the difference that the concepts in the open set are typically assumed to come from categories that are not peers of the ones in the closed set. It has to be noted that unlike ND, the closed set class labels are provided during training, and the model is expected to classify the input data into these classes as well as identifying closed vs. open sets at the inference time. Having access to the class labels often makes OSR and OOD detection an easier task than ND.
% %When performing OOD detection, two different datasets are employed - the closed set and the open set. The absence of data labels as an additional information source during training separates ND from OSR and OOD techniques, which possess this capability. This attribute makes ND a more challenging undertaking. 

% Robustness  against adversarial attacks is a key requirement in the real world model development. Adversarial attacks are the imperceptible input perturbations that are designed to cause the model to make incorrect predictions \cite{szegedy2013intriguing,goodfellow2014explaining,akhtar2018threat}. It is well known that the standard training makes the models vulnerable to such attacks in the classification problem \cite{madry2017towards,wong2020fast,zhang2019theoretically}, and in particular in the anomaly detection \cite{chen2021atom,fort2022adversarial}.  This issue is more significant in anomaly detection as it violates the main premise of such methods, which was to guard the model against unknown concepts in safety-critical applications \cite{chen2020robust}. Anomaly detection methods have not been successful in achieving ideal robust detection rates despite attempts to make them adversarially robust \cite{azizmalayeri2022your,lo2022adversarially,chen2020robust,shao2020open,shao2022open,bethune2023robust,goodge2021robustness,chen2021atom}. 

% %The issue is also more challenging to tackle in the case of anomaly detection, as the anomalous patterns are often very diverse and unknown a priori during training. This makes adversarial training, which is the standard defence against such attacks by augmenting the data with adversarial perturbations, impossible. That is, the straightforward application of the adversarial training on the normal data would make the model robust against only the normal data. This happens because the model do not encounter examples of adversarial perturbations on anomalous data during training, which results in poor adversarial generalization on the anomalous data.

% \input{Figures/First_Figure}

% %Despite several attempts to bring adversarial robustness to anomaly detection, the detection rates are still far from being ideal \cite{azizmalayeri2022your,lo2022adversarially,chen2020robust,shao2020open,shao2022open,bethune2023robust,goodge2021robustness,chen2021atom}. We note that as the anomalous patterns are often very diverse \cite{salehi2021unified}, and unknown a priori during training, adversarial training becomes less effective when applied naively in training of many existing anomaly detection methods. This stems from the fact that the model would not be able to generalize to resist against adversarial perturbations that are associated with the anomaly data, as such perturbations have not been presented to the model during the training. For this reason, recent robust anomaly detection methods commonly leverage a set of outlier samples during training \cite{azizmalayeri2022your,chen2020robust,chen2021atom}. This technique is called outlier exposure (OE) \cite{hendrycks2018deep}.

% %While many methods have significantly performance on commonly used benchmark datasets, which assume in-distribution (ID) and out-of-distribution (OOD) data to be benign, the robustness of detection models against adversarial instances continues to be suboptimal. 
% %For instance, the performance of the SOTA robust ND model on CIFAR-10 is 50\% less than the result of the SOTA ND model on 
 


% %Recently, there has been increasing interest in developing robust models for anomaly detection, and several methods have been proposed. However, these methods have several limitations, as most of them are designed for specific settings and cannot be easily adapted to other modes. For instance, while ATD have shown promising results in OOD, it exhibit a strong inductive bias towards labeled data, which renders them unsuitable for use in the no data-label (ND) setting.

% %Another drawbacks of the proposed methods is their limited applicability to diverse datasets. They are only effective in dealing with simple datasets and cannot be used in practical or industrial benchmarks. It is important to mention that there is currently a lack of a robust anomaly detector in the medical imaging domain, which is an urgent issue that needs to be addressed.

% %To this end, we investigated several strategies towards this goal. Specifically, we study the effect of transfer learning and adaptive outlier exposure in achieving robust anomaly detection. Transfer learning, involving the utilization of a pre-trained model for downstream tasks, is a subject of investigation across several domains, encompassing image classification, object detection, segmentation, among others. In this study, we intend to investigate the efficacy of transfer learning from a robust model in achieving robust anomaly detection, representing a pioneering exploration in this area.

% Adversarial training, which is the augmentation of training samples with adversarial perturbations, is among the best practices in making models robust. However, it is less effective in anomaly detection as the anomalous patterns are not known during training, so one cannot train the model with adversarial perturbations associated with anomalies. For this reason, recent robust anomaly detection methods use outlier exposure (OE) in combination with adversarial training to tackle this issue \cite{azizmalayeri2022your,chen2020robust,chen2021atom}. In OE, outlier samples that are typically obtained from other datasets are leveraged during training. Our key insight is that: %Many top-performing out-of-distribution (OOD) detection techniques, both in common benign benchmarks and adversarial settings, often employ OE as a key component of their approach \cite{fort2021exploring,deecke2021transfer,reiss2021panda,mirzaei2022fake,liznerski2022exposing}. 

% {\it The set of outliers in OE methods need to be ``diverse'', ``near-distribution'', and conceptually differentiable from the normal samples, for the adversarial training to be effective in robust anomaly detection.}

% The need for diverse outlier samples is often associated with the increased sample complexity in adversarial training. \cite{schmidt2018adversarially}. By the near-distribution  outliers, we mean such data possess  semantically and stylistically related characteristics to that of the normal set. If the outliers are not near-distribution, the classification boundary would be misplaced in the input space, causing a distribution shift on the adversarial perturbations of the outlier samples compared to that of the real anomalies. We provide a comprehensive assessment of these claims in the ablation studies.  
% %Previous studies have demonstrated the effectiveness of this technique in anomaly detection.

% %For example, Ruff achieved impressive AUROC scores of 99.2 and 87.5, respectively, when CIFAR-10 was utilized as the closed set, and CIFAR-100 and SVHN were employed as OE datasets. These results suggest that near-distribution OE could be more effective for anomaly detection. 

% %Numerous studies have demonstrated that the majority of detection models exhibit a decline in performance under minor distribution shifts in either the open or closed set data [[... citing S. Y. Li papers here ...]]. In this paper, we focus on adversarially perturbed test samples, and investigate effective remedies to decrease the mentioned decline in performance of ND, OSR, and OOD detection under evasion attacks. Our main goal is to come  up with a set of unified strategies that are effective and agnostic to the baseline model. To highlight the difficulty of robust OOD detection, note that state-of-the-art clean AUC for CIFAR-10 vs. CIFAR-100 is around 98\%, whereas it is 38\% in an adversarial setting. Our key insight to improve such results is to take a data-centeric approach. We note that the adversarial vulnerability of these detection methods stems primarily from unknown nature of the adversarial perturbations in the open set classes. We address this problem by estimating near-distribution open set samples, by employing a guided diffusion-based text-to-image generation approach. In certain aspects, our task involves image-to-image translation, conditioned on both the input text and input image. The input text is automatically extracted from a language model, conditioned on the name of the normal class combined with certain negative adjectives to make the generated image deviate from the normal class.

% %In this paper, we start by revealing key insights that the effectiveness of the outlier exposure technique is contingent on the distribution of the exposed outliers. Our study involved evaluating OOD detection models that integrate the outlier exposure technique into their pipeline, using the CIFAR-10 dataset for the training. As the results illustrate, it is more effective when the distribution of exposed outliers exhibits semantically and stylistically related characteristics to that of the normal set. 

 
% Motivated by this, we suggest an adaptive outlier exposure technique utilizing guided diffusion models as a substitute for the prevalent random sampling method in the literature. We assume that the title(s) of the normal classes are known during training. Such titles are modified slightly through exploring the semantically rich embedding space generated by the Word2Vec model \cite{mikolov2013efficient}                                 to identify negative adjectives of a class, such as ``broken'' for the ``screw'' class, or word replacements such as ``nail'' for the ``screw'' class. The modified title is then given as a prompt to a pre-trained text-to-image generative model that is conditioned on a normal image to generate outliers for OE. Finally, a classifier is adversarially trained to distinguish generated outliers from the normal samples.

% The key idea here is that crafting outliers is often more manageable through the language, compared to directly making edits in the image space. Note that the latter may not necessarily turn a normal image into an anomalous one, while the former is better suited for this purpose. In addition, by searching for the words with the closest meaning to the normal titles, and also conditioning on the normal image, the generated outlier would be near-distribution. Leveraging pre-trained text-to-image generative models also helps in making diverse samples.
% The empirical results of ND setup on various tiny, medical, and industrial datasets, and also the generalization of the method to OOD detection and OSR setups, show that our method, RODEO, makes a huge improvement in the adversarial AUC under various attacks. 

% %The results of our study demonstrate that utilizing adaptive OE in the training process can significantly improve the robustness of an OOD detector. 
% %Our investigation examines the performance of RODEO in various OOD detection environments, encompassing common benchmarks and adversarial tasks. Our testing involves unlabeled one-class, unlabeled multi-class, and labeled multi-class settings. Significantly, we are the first to demonstrate all three settings under a single framework in the field of robust OOD.
% %Furthermore, we include medical and industrial datasets to emphasize the practical significance of our work. Overall, our results demonstrate that our method, RODEO, outperforms baseline methods on all evaluated datasets.
% Our key results and contributions are:

% \begin{itemize}
%     \item We propose a novel method, adversarial training with adaptive outlier exposure, that allows for the efficient integration of auxiliary outlier data, resulting in robust OOD detection, ND, and OSR. Our method has achieved state-of-the-art performance by increasing the AUROC up to 40\%.
 
%     \item 
%  We extensively evaluate RODEO in various OOD detection environments, encompassing common benchmarks and adversarial tasks. Our testing involves unlabeled one-class, unlabeled multi-class, and labeled multi-class settings. Significantly, we are the first to demonstrate all three settings under a single framework in the field of robust OOD detection.
% %  \item  Furthermore, our work involves an exploration of robust pretraining for the task of robust OOD detection. Notably, we have demonstrated for the first time that pre-trained adversarially robust neural networks on the ImageNet dataset can be leveraged to improve the results.
%  %    \item
%  % We provide theoretical insights on why outlier mining with high boundary scores benefits sample efficiency.
% \end{itemize}

% %We have proposed a new outlier exposure technique through text-to-image guided diffusion models, which facilitates the efficient use of outlier exposure conditions on the normal dataset. The proposed technique promotes the learning of a decision boundary between in-distribution (ID) and out-of-distribution (OOD) data, thereby improving the robustness of OOD detection.
\end{itemize}

==> Tables/Method.tex <==
\section{Method}



\subsection{Proposed Pipeline}
To develop a robust OOD detection model, the outlier exposure technique appears to be crucial \cite{chen2021atom}, otherwise, the model lacks information about outlier data, leaving it highly vulnerable to adversarial attacks targeting OOD data. Our goal is to generate diverse and near-distribution outliers that can act as proxies for real outliers during testing. Although some studies have attempted to generate useful outliers, they often lack diversity and fail to maintain proximity to the distribution. This issue largely arises from neglecting certain aspects of the normal data distribution. These studies typically operate strictly within the image domain, using a generator (either GAN or Diffusion) to craft OOD samples. However, our results suggest that considering text information is crucial. By utilizing both text and image information to generate adaptive OE, we can guide the model to establish a more accurate decision boundary.

 In the following sections, we will provide a detailed description of the three primary stages of our methodology: generation, training, and testing, along with their respective elements. \\ \\

%  \subsection{Proposed Pipeline}
% Building on established intuitions, we propose employing a pre-trained diffusion model to generate diverse and high-quality near-distribution OOD samples. To be more precise, assuming that we have labels for a normal dataset (e.g., "Dog"), we use a simple text encoder to extract words that are semantically similar to the normal labels but are different from normal ones (e.g., "Wolf"). Using these near out-of-distribution words, we guide the generative model, to generated near outlier exposure data. condition on normal images.
%  In the following sections, we will provide a detailed description of the three primary stages of our methodology: generation, training, and testing, along with their respective elements. \\ \\

 
 \subsubsection{Generation Step}
% In the following sections, we will provide a detailed description of the three primary stages of our methodology: generation, training, and testing, along with their respective elements. \\ \\
\textbf {Conditioning on Text:}
Employing a text extractor model and given the labels of the normal data, we can identify words closely related to them. We utilize Word2Vec, a simple and popular model, to obtain the embeddings of the normal labels (e.g. \textit{"screw"}) and subsequently retrieve their nearest labels (e.g. \textit{"nail"}). In the next step, we remove the extracted labels that are close to the normal labels and are still in-distribution with high probability. We then add some texts containing negative attributes of the normal data labels to the extracted set (e.g. \textit{"broken screw"}). The union of these two sets of labels forms the final set of prompts used to guide the image generation process. More details about choosing the nearest labels and negative adjectives are available in Appendix.\\ \\
\textbf{Conditioning on Image:} 
We utilize the GLIDE model as our generator. Our aim is to generate near Outlier Exposure (OE) that exhibits similar features to those in normal images. As a result, we initiate the diffusion process from a random step $t_{init} \sim \mathcal{U}([T_0, T])$, rather than beginning from $t=0$. This approach is crucial to prevent the diffusion process from starting with pure noise, which would result in the loss of information from the original normal image. Then starting from step $t_{init}$ of the reverse diffusion process of GLIDE, we use this prompt and CLIP guidance to generate near-distribution OOD sample $\hat{x}_0$ from the normal sample by progressively repeating the following reverse diffusion step:


$\quad \quad \hat{x}_{t-1} \sim \mathcal{N} ( \mu_{Glide}(\hat{x}_t|c) + s \cdot \Sigma_{Glide}(\hat{x}_t|c)\cdot \nabla_{\hat{x}_t} (f_{clip}(\hat{x}_t) \cdot g_{clip}(c)) \ , \ \Sigma_{Glide}(\hat{x}_t|c) \ )$\\ \\
\textbf{GLIDE:} 
In Appendix \ref{two_type_ood}, we discussed how OOD data can be divided into two categories pixel- and semantic-level. Our need for diverse OOD data motivates our preference for generative models that can create both pixel-level and semantic-level OOD data. Among the many advanced text-to-image models available, GLIDE distinguishes itself by operating in pixel space, as opposed to latent space utilized by other models. Therefore, GLIDE is a suitable choice as it uses a diffusion model applied at the pixel-level to generate images from prompts. This allows GLIDE to generate OOD samples that differ not only in their semantic content but also in their local appearance (pixel-level OOD samples) and thus create diverse OOD data. Generating pixel-level OOD samples can be challenging with latent space-based generative models. In the appendix, we have also compared the outputs of GLIDE with those of other feasible alternative generative models. It's worth noting that GLIDE has been trained on only one percent of the number of training samples compared to other state-of-the-art (SOTA) text-to-image models (e.g., Stable Diffusion).




% Therefore, considering GLIDE's comparable ability in inducing semantic shifts, we select it as our preferred choice for outlier generation.


% GLIDE is a suitable choice as it uses a diffusion model applied at the pixel-level to generate images from natural language prompts. This allows GLIDE to generate OOD samples that differ in their local appearance, which is particularly important for pixel-level OOD detection. Compared to other state-of-the-art text-to-image models that mostly work at the embedding level, GLIDE's ability to generate images at the pixel-level makes it a better choice for our purposes.


%  Among the many advanced text-to-image models available,GLIDE, distinguishes itself by operating in pixel space, as opposed to latent space utilized by other models. While latent space models offer advantages such as reduced complexity and potential proficiency in semantic shifts, we deliberately opt for GLIDE as our outlier generator. Its operation in pixel space enables the generation of outliers with pixel-level flaws, a crucial form of near-distribution shift for various applications, including industrial and medical settings where pixel-level anomalies are prevalent. Achieving this type of shift can be challenging with latent space models. Therefore, considering GLIDE's comparable ability in inducing semantic shifts, we select it as our preferred choice for outlier generation.

 
 % Building on established intuitions, we propose employing a pre-trained diffusion model to generate diverse and high-quality near-distribution OOD samples. These samples will serve as exposure during the training of robust OOD detectors. Instead of image-conditioned diffusion models with limited OOD distribution control, we leverage class labels (access to class names is not a stringent requirement even in real-world situations) to identify near-distribution OOD labels in a natural language context, a simpler task than searching in image space. Then, we transform these text-based findings into image samples using powerful text-to-image diffusion models that have driven significant advancements in real-world machine learning applications.

 
% \paragraph{Guiding Detectors through robustness with Adaptive Outlier Exposure:} Building on established intuitions, we propose employing a pre-trained diffusion model to generate diverse and high-quality near-distribution OOD samples. These samples will serve as exposure during the training of robust OOD detectors. Instead of image-conditioned diffusion models with limited OOD distribution control, we leverage class labels (access to class names is not a stringent requirement even in real-world situations) to identify near-distribution OOD labels in a natural language context, a simpler task than searching in image space. Then, we transform these text-based findings into image samples using powerful text-to-image diffusion models that have driven significant advancements in real-world machine learning applications.
% In the subsequent sections, we outline the primary elements of our comprehensive approach aimed at overcoming the challenges of robust anomaly detection.
% In this order instead of starting from step $t=0$ and initializing with random noise, we initialize the reverse process of GLIDEs diffusion model from a random step $t_{init} \sim \mathcal{U}([T_0, T])$ using a normal data point $x_i$ sampled from in-distribution training dataset as $\hat{x}_{t_{init}}$. We also sample an OOD prompt c from near distribution prompts corresponding to label($y_i$) of the normal sample $x_i$.

% \subsubsection{Note *   }
 
% Robust anomaly detection has shown to be a challenging task in different settings [refs], particularly in the absence of explicit assumptions and inductive biases regarding training and test time conditions. In the one-class setting, adversarial training poses an even greater challenge in achieving robustness, as the absence of supervised classification during training further complicates the task. In the subsequent sections, we outline the primary elements of our comprehensive approach aimed at overcoming the challenges of robust anomaly detection across different settings.

% We assume that an in-distribution dataset $D_{in}$ of $(x_{in}, y_{in})$ is available during training, where $x$ represents the input data   and $y_{in} \in Y_{in} := \{i_1, \dots, i_k\}$ represents the class label. Additionally, let $D_{out}$ represent an out-of-distribution dataset of $(x_{out}, y_{out})$ pairs, where $y_{out} \in Y_{out} := \{o_1, \dots, o_M\}$ and the intersection of $Y_{in}$ and $Y_{out}$ is  $ \emptyset$. 
% \input{Figures/Third_Figure}
\input{Figures/Samples}
\input{Figures/Second_Figure}

\subsubsection{  Training Step }

\textbf{Adversarial Training:} During training we have access to an in-distribution dataset $\mathcal{D}^{in}$ of pairs $(x_i, y_i)$ where $y_i \in \{1, ..., K \}$ and we augment it with generated adaptive dataset $D^{aug}$ of pairs $(\hat{x}_i, K+1)$ as outlier exposures to obtain $\mathcal{D}^{train} = \mathcal{D}^{in} \cup D^{aug}$. Then we adversarialy train a classifier $f_{\theta}$ with standard cross-entropy loss $\ell_{\theta}$:$ \quad 
\quad \quad \min_{\theta} E_{(x,y) \sim \mathcal{D}_{train}} \ \ \max_{|| x^* - x ||_{\infty} \leq \epsilon} \ell_{\theta}(x^*, y)
$

with minimization and maximization done respectively by optimiser and PGD. For evaluation purposes, we utilize a dataset $D^{test}$ that consists of both in-distribution and out-of-distribution samples. 
 
\subsubsection{  Testing Step }

\textbf{Adversarial Testing:} During test time We utilize the $K+1$'th logit of $f_{\theta}$ as the OOD score, which corresponds to the class of outliers in the training dataset.  For the evaluation of our model, as well as other methods, we specifically target both in-set and out-set samples with an end-to-end  PGD attack. Our objective is to cause detectors to produce erroneous detection results by decreasing OOD scores for outlier samples and increasing OOD scores for normal samples. We set the value of $\epsilon$ to $\frac{8}{255}$ for low-resolution datasets and $\frac{2}{255}$ for high-resolution ones. For the models' evaluation, we use a single random restart for the attack, with random initialization within the range of $(-\epsilon, \epsilon)$ , and perform 100 steps. Furthermore, we select the attack step size as $\alpha=2.5 \times \frac{\epsilon}{N}$.
In addition to the PGD attack, we have evaluated models using AutoAttack \cite{croce2020reliable}, a recently introduced method designed to enhance robustness evaluation by implementing more potent attacks. Moreover, we have assessed models in the context of a black-box setting \cite{guo2019simple}.
We have provided details about the evaluation metrics used in our study in appendix. For additional information on the dataset and implementation, please refer to the appendix section.



% our method proposes a general framework of outlier exposure for different settings of out-of-distribution detection and demonstrates a superior adversarial robustness to task-specific state of the art algorithms. in addition to sub-optimal performance of algorithms of robust OOD detection in setting like one-class anomaly detection [refs], open-set recognition [refs] and OOD detection comparing to our results, main shortcomings of these algorithms is using task dependant inductive biases for targeted task which weakens the generalization of their abilities to other important settings of safety and robustness.

% In order to improve the robustness of an OOD detector without any explicit assumption on properties of closed-set or open-set distributions, we use a dataset of K classes in-distribution data like $\mathcal{D}_{train}$ with a supervised approach and augment its label space with a new class called outliers with label K+1 and corresponding data points $\mathcal{D}_{aug}$ generated by our adaptive outlier generator. then we adversarially train a classifier on the augmented dataset. for evaluations of OOD detection performance, we use logits corresponding to outliers class as anomaly score.

% In adversarial attacks on anomaly detection performance of neural networks with an additional exposure class, a basic PGD attack on cross-entropy loss, given by $x^{t+1} = x^t + \alpha \cdot \text{sgn}(\ell_{\theta}(x^t,y))$, proves inadequate, as perturbations between in-distribution classes do not impair OOD detection. Instead, an attack based on the anomaly score is employed, represented by 
% $$
% x^{t+1} = x^t + \alpha \cdot t \cdot \text{sgn}(\ell_{\theta}(x^t,K+1) ) \ \ \ \ \ \text{where} \ \ \ 
% t= \left\{
% \begin{array}{ll}
%       +1 \ \ \ \ \ \ \ y = K+1 \\
%       -1 \ \ \ \ \ \ \ y \in \{1, ..., K \} \\
% \end{array}
% \right. 
% $$
% This approach for attacks aims to increase the last logit (anomaly score) for in-distribution samples and decrease it for exposure samples. Therefore, the resulting loss function for adversarial training is as follows:
% $$
% \min_{\theta} E_{(x,y) \sim \mathcal{D}_{train}} [ \min_{\delta \in \Delta} \ell_{\theta}(x+\delta, K+1) ] + E_{(x,y) \sim \mathcal{D}_{aug}} [ \max_{\delta \in \Delta} \ell_{\theta}(x+\delta, K+1) ]
% $$
% the flexibility of using outlier exposure in a discriminative detection method makes it suitable for different setups of out-of-distribution detection. for unlabeled one-class Novelty Detection which is a hard setup to be solved by discriminative solutions, OE turns the task into a simple binary classification and similarly, it easily fits into OSR and OOD settings. also, its generalization to consider different assumptions on these tasks (e.g. unlabeled multi-class OOD/OSR/ND[refs] or multi-label setups [refs] ) is evident. In its simplicity, our results show that combining outlier exposure with adversarial training can outperform SOTA setup-specific OOD Robustness methods.



% \subsubsection{Guiding Detectors through robustness with Guided Diffusion Models}
% Building on established intuitions, we propose using a pretrained diffusion model to generate high-quality near-distribution OOD samples for training robust OOD detectors. Instead of image-conditioned diffusion models with limited OOD distribution control, we leverage class labels (access to class names is not a stringent requirement even in real-world situations) to identify near-distribution OOD labels in natural language context, a simpler task than searching in image space. Then, we transform these text-based findings into image samples using powerful text-to-image diffusion models that have driven significant advancements in real-world machine learning applications.

% \textbf{Near-Distribution Prompting:} When generating near-distribution OOD samples, two types of shifts are considered: semantic and pixel-level shifts. Semantic shifts involve altering samples' meaning while retaining the original dataset's style, while pixel-level shifts introduce visual perturbations. Examples include transforming a shoe to a bag in Fashion-MNIST (semantic) and adding defects like cracks in MVTec dataset images (pixel-level). Our model uses word embeddings, such as WordNet, to identify near-distribution labels for generating OOD samples (e.g., "broken screw" or "nail" for the "screw" class). We use a a batch of prompts for each class containing both types of prompts. This approach accommodates various OOD variations and helps to effectively demonstrate the boundaries between in-distribution and OOD data.


% \textbf{In-Distribution Guidance:} To concurrently utilize textual information and in-distribution images while retaining the style of the training distribution and keeping OOD samples close, one option is to develop custom diffusion models that incorporate both guidance types. However, a simpler alternative is using pretrained text-to-image models. By employing in-distribution images as the starting point for the reverse diffusion process, instead of conditioning on their embeddings or sampling noise at timestep 0, we can mutate these images under the guidance of a prompt to generate near-distribution samples. Figure \ref{fig:Diff_Plot} offers a visual representation of this method.



%Algorithm \ref{alg:RODEO} presents the entire algorithm, encompassing all components of our approach.


% With the GLIDE model and both types of prompts, we generate near OOD data by injecting in-distribution images at varying middle steps of the reverse diffusion process, depending on the prompt type. As noted in [https://arxiv.org/abs/2206.00070], a dynamic transition point in the reverse diffusion process exists, shifting from producing distorted images to denoising them. In light of this observation, initiating the process at earlier stages is more effective for semantically-shifted prompts to maintain style while modifying semantics. Conversely, starting at later stages is appropriate for pixel-level shifts, minimizing substantial semantic alterations and emphasizing pixel-level disturbances. This strategy ensures the generated near OOD data aligns with the desired characteristics based on the prompt type. 
% \scalebox{0.7}{
%     \begin{algorithm}[H] 
%         \SetAlgoLined
%     		\KwIn{$\mathcal{D}_{\text{in}}$, $enc_{text}$, \mu_{Glide}, \Sigma_{Glide}, $f_{clip}$, $g_{clip}$, $f_\theta$, $K$, $T_0$, $T$ \tcp*{ $T_0 \in [0.3T, 0.6T]$ } }
    		
%             \KwOut{$\hat{f}_{\theta}$} 
%             \tcp{Near-Distribution OOD Prompt Search}
%             \For{$(i, label) \in Y$}{
%                   $Prompts[i] \leftarrow enc_{text}.KNN(label) \cup Append(NegativeAdjectives[label], label)$ \\
%                   $Prompts[i] \leftarrow Prompts[i].Filter( enc_{text}.MinDist(Prompt  ,  Y \ \backslash \ label) > \epsilon$ )
%             }
%             \tcp{Adaptive Exposure Generation}
%             \For{$(x_i, y_i) \in \mathcal{D}_{\text{in}}$}{
%                           $c \sim \mathcal{U}(Prompts[y_i])$ \\
%                           $t_{init} \sim \mathcal{U}([T_0, ..., T]$ \\
%                           $\hat{x}_{t_{init}} = x_i$ \\
%                           \For{$t=t_{init} , ... , 0$} {
%                             $ \hat{\mu}(\hat{x}_t | c) = \mu_{Glide}(\hat{x}_t|c) + s \cdot \Sigma_{Glide}(\hat{x}_t|c)\cdot \nabla_{\hat{x}_t} (f_{clip}(\hat{x}_t) \cdot g_{clip}(c)) $ \\
%                             $ \hat{x}_{t-1} \sim \mathcal{N}( \ \hat{\mu}(\hat{x}_t | c) \ , \  \Sigma_{Glide}(\hat{x}_t|c) \ ) $ \\
%                           } \\
%                           $\mathcal{D}_{\text{exposure}} \leftarrow \mathcal{D}_{\text{exposure}} \cup \{ (\hat{x}_0, K+1) \}$
%                     }
    
%             $\mathcal{D}_{\text{train}} \leftarrow \mathcal{D}_{\text{in}} \cup \mathcal{D}_{\text{exposure}}$ \\
%             $ \hat{f}_{\theta} \leftarrow \text{AdversarialTraining}(f_{\theta}, \mathcal{D}_{\text{train}}) $
    
    
            
            
%             \caption{RODEO: Adv. Training with Adaptive Exposure Dataset}
%             \label{alg:RODEO}
%     \end{algorithm}
% }

% \textbf{Distribution of Outliers Matters} \{explain why adaptive is important, importance of near distribution and why in pixel space not in latent\}

% given an ideal encoder e:$\mathcal{X} \rightarrow \mathcal{Z}$ and an exposure dataset with distance coefficient r which measures the distance to in-distribution boundaries (r=1 perfect near OOD and r=0 far OOD ) with i.d. features ($0 \leq r \leq 1$) ,we define data models in feature space $\mathcal{Z}$ in following manner:

% training setting under adaptive exposure ($y \overset{\mathrm{u.a.r.}}{\sim} \{-1,+1\}$):

% \begin{equation}
% D_{train}(z,y)= \left\{
% \begin{array}{ll}
%       z_1 \sim \mathcal{N}(+1, u^2) , z_2, ..., z_{d+1} \overset{\mathrm{i.i.d.}}{\sim} N(\eta, 1) & y = +1 \\
%       \tilde{z}_1 \sim \mathcal{N}(r-1, v^2) , \tilde{z}_2, ..., \tilde{z}_{d+1} \overset{\mathrm{i.i.d.}}{\sim} N(\eta.(r-1), 1) & y = -1 \\
% \end{array}
% \right. 
% \end{equation}

% testing ($y \overset{\mathrm{u.a.r.}}{\sim} \{-1,+1\}$):

% \begin{equation}
% D_{test}(z,y)= \left\{
% \begin{array}{ll}
%       z_1 \sim \mathcal{N}(+1, u^2) , z_2, ..., z_{d+1} \overset{\mathrm{i.i.d.}}{\sim} N(\eta, 1) & y = +1 \\
%       \tilde{z}_1 \sim \mathcal{N}(-1, u^2) , \tilde{z}_2, ..., \tilde{z}_{d+1} \overset{\mathrm{i.i.d.}}{\sim} N(-\eta, 1) & y = -1 \\
% \end{array}
% \right. 
% \end{equation}

% in ideal case which is access to real datas from -1 class of test setting a classifier like $w=[0,\frac{1}{d}, ..., \frac{1}{d}]$ achieves high accuracy ($>99\%$ ) but low  adversarial accuracy ($<1\%$) [Robustness May Be at Odds with Accuracy Tsipras et.al.].

% also in training setting a classifier like $\tilde{w}=[0,\frac{r}{d}, ..., \frac{r}{d}]$ achieves high accuracy with low adversarial accuracy:

% standard accuracy:

% $$ Pr[ f_{avg}(x) = y] = Pr[sign(\tilde{w}x) = y] = $$

% $$ = Pr[\frac{r.y}{d} \sum_{i=1}^{D} \mathcal{N}(\eta, 1) I [ y==+1 ] + \mathcal{N}(\eta.(r-1), 1) I [ y==-1 ] > 0] = $$

% $$ = \frac{1}{2} ( Pr[ r\mathcal{N}(\eta, \frac{1}{d}) > 0] + Pr[ r\mathcal{N}(\eta(1-r), \frac{1}{d}) > 0 ]) $$

% which is $>99\%$ when $ \eta \geq \frac{3}{\sqrt{d}.(1-r)}$.


% \\
% Adversarial accuracy for $\epsilon \geq 2\eta$:
% $$
% \min_{  || \delta ||_{\infty} \leq \epsilon } Pr[ sign(\tilde{w}(x+\delta)) = y  ] \leq \frac{1}{2} (Pr[r\mathcal{N}(\eta,\frac{1}{d}) - \epsilon > 0] + Pr[ r\mathcal{N}(\eta(r+1), \frac{1}{d}) - \epsilon > 0 ]) = 

% $$
% = \frac{1}{2} (Pr[r\mathcal{N}(-\eta,\frac{1}{d}) > 0] + Pr[ r\mathcal{N}(-\eta(r+1), \frac{1}{d}) > 0 ])
% $$

% which is $<1\%$.


% we now show training signals is in direction of non-robust feature regularization. so we show that similarly to training with real outlier data and classifier head with weights  $w$, gradients of minimizing loss of a linear classifier with weights $\tilde{w}$ on exposure dataset guides the feature embedding function to pay less attention to non-robust features.
% we see that similarity degree of effect of
% the training signals obtained from the exposure adversarial
% loss from the perspective of non-robust feature regularization are related to primary task by the parameter $r$.

% Magnitude:
% $$
% E \left[\frac{\partial \ell(\tilde{w})}{\partial \tilde{z}_i^{adv}} \right] = E \left[\tilde{w}_i(\sigma(\tilde{w} z^{adv}})-\frac{y+1}{2}) \right] = E \left[\frac{r}{d}(\sigma(rwz^{adv})-\frac{y+1}{2}) \right] =
% $$

% $$
% = r.E \left[ \frac{1}{d}(\sigma(wz^{adv})-\frac{y+1}{2}) \right] = r.E \left[ \frac{\partial \ell(w)}{\partial z_i^{adv}} \right]
% $$

% Direction:

% $\tilde{z}^{adv}$ can be approximated by $ \tilde{z} + \lambda . sign(\nabla_{\tilde{z}} \ell (w) )$ for  $ \eta < \lambda < 1$:

% $$
% E \left[ \tilde{z}_{i}^{adv} \right] = E \left[ \tilde{z}_i + \lambda . sign(\frac{\partial \ell(\tilde{w})}{\partial \tilde{z}_i}) \right] = \eta(1-\frac{r}{2})y + \eta \frac{r}{2} + \lambda.E \left[ sign(\tilde{w}_i( \sigma(\tilde{w}\tilde{z}) - 
% \frac{1+y}{2} )) \right] = 
% $$

% $$
%  = \eta(1-\frac{r}{2})y + \eta \frac{r}{2} - \lambda y
% $$

% $$
% \rightarrow \ \ \ \  sign(E \left[\frac{\partial \ell(\tilde{w})}{\partial \tilde{z}_i^{adv}} \right]) = sign(E \left[ \tilde{z}_{i}^{adv} \right]) \ \ \ \ \ for \ \ \ \ \ 2.\eta < \lambda
% $$ 



% Motivated by this, recent works \cite{chen2020robust,azizmalayeri2022your} have proposed robust OOD detection models using outlier exposure.
% However, as illustrated in Figure\ref{fig:Comparison_Plot}, their performance is highly dependent on the distance between the distribution of the exposed outliers and the target dataset. Our experimental results (see Table \ref{Table:Ablation_1}) suggest that vanilla outlier exposure (OE) methods may underperform when the exposed dataset is significantly different from the normal data distribution. For example, as results illustrate, using ImageNet as an outlier exposure dataset is highly beneficial when the normal dataset is CIFAR-10, due to the relatively small distance between the two distributions. However, when the normal dataset is MNIST, which is relatively far from ImageNet in terms of distribution, the use of ImageNet as an outlier exposure dataset has less of an effect. Additionally, our theoretical insights highlight the potential benefits of utilizing near outlier exposures, especially within adversarial contexts. This observation motivates us to propose an adaptive technique for generating near-outlier exposures. To achieve this, the data generation technique must be conditioned on the information from the distribution of the normal set. While some previous works have proposed conditional generation techniques to create more adaptable outlier exposures compared to traditional methods (which used a fixed dataset for outlier exposure), they failed to achieve satisfactory results. This is because they only considered information in the image domain for conditioning. In contrast, we leveraged all available information in the normal set, including both images and text. Our ablation study demonstrated that excluding any of this information leads to a decrease in performance.

==> Tables/Multi-Class.tex <==
 

\begin{table*}[h ]
\centering
\caption{AUROC scores for Multi-class settings under PGD adversarial attack with 100 steps and $ \epsilon = \frac{8}{255} $. The best and second-best results are highlighted in bold and
underlined format respectively in each row. The detailed results of the experiments can be found in the Appendix.}
\begin{subtable}{1\textwidth}

\BlankLine
\centering
\subcaption{Out-of-distribution detection}
\resizebox{0.7\linewidth}{!}{\begin{tabular}{ll*{9}{c}} 
\specialrule{1.5pt}{\aboverulesep}{\belowrulesep}
\noalign{\smallskip}

   \multirow{3}{*}{\large{In-Dataset}} & \multirow{3}{*}{\large{Attack}}  &\multicolumn{8}{c}{Method}\\
    \cmidrule(lr){3-10}  
    
  &&\multirow{1}{*}{OpenGAN}&\multirow{1}{*}{ViT} & \multirow{1}{*}{ATOM} &\multirow{1}{*}{AT} & \multirow{1}{*}{OSAD} & \multirow{1}{*}{ALOE}& \multirow{1}{*}{ATD} &  RODEO&
   \\
  & &\cite{kong2021opengan}& \cite{dosovitskiy2020image} & \cite{chen2021atom} & &\cite{shao2022open} & \cite{chen2020robust} & \cite{azizmalayeri2022your}  &  (Ours)    
 \\
\noalign{\smallskip}
 \hline
\noalign{\smallskip}
% capsnet: 1911.08616
% rest: ARAE 97.5	\_	64.1	73
 
\multirow{2}{*}{CIFAR10}
&\multirow{1}{*}{\centering Clean}&\underline{97.1}&\textbf{99.5}& 97.8 & 80.5&82.7&84.3&94.3 & 93.2 \\&\multirow{1}{*}{\centering PGD-100}&26.6&0.0&  6.0  &20.8&25.1&28.7&\underline{69.3}& \textbf{70.4}\\

\noalign{\smallskip}
 \hline
\noalign{\smallskip}
 
\multirow{2}{*}{CIFAR100}
&\multirow{1}{*}{\centering Clean}&\textbf{95.8}&\underline{95.1}& 91.6 & 70.0&61.5&79.3&87.7& 88.1&   \\&\multirow{1}{*}{\centering PGD-100}&8.8&0.0&5.4 &13.6&21.6&26.4&\underline{55.3}& \textbf{66.4}  \\

 \specialrule{1.5pt}{\aboverulesep}{\belowrulesep}
\end{tabular}}
\end{subtable}

\bigskip
 
\begin{subtable}{1\textwidth}


\centering
\caption{Open-set recognition}
\resizebox{0.7\linewidth}{!}{\begin{tabular}{ll*{9}{c}} 
 \specialrule{1.5pt}{\aboverulesep}{\belowrulesep}
 \noalign{\smallskip}



   \multirow{3}{*}{\large{Dataset}} & \multirow{3}{*}{\large{Attack}}  &\multicolumn{6}{c}{Method }  
     \\   
    \cmidrule(lr){3-9}  


  &&\multirow{2}{*}{OpenGAN}&\multirow{2}{*}{ViT}&\multirow{2}{*}{AT} & \multirow{2}{*}{OSAD} & \multirow{2}{*}{ALOE}& \multirow{2}{*}{ATD} &  RODEO  &
   \\
 
  & && &  &      &  &   &    (Ours)     
 \\
 
\noalign{\smallskip}
 \hline
\noalign{\smallskip}



% capsnet: 1911.08616
% rest: ARAE 97.5	\_	64.1	73

\multirow{2}{*}{MNIST} &Clean&\textbf{99.9}&92.4&80.2 & 74.3   & 79.5& 68.7 &\underline{97.2}
\\ & PGD-100&13.3&4.2&36.2 & 47.1   & 38.2& \underline{56.7} & \textbf{88.8}
\\ 
      \cmidrule(lr){1-1} \cmidrule(lr){2-2} 
    \cmidrule(lr){3-10} 


\multirow{2}{*}{Fashion-MNIST} &Clean&\textbf{98.4}&87.6&72.5 & 68.0  & 72.6& 59.6 & \underline{87.7}
\\ & PGD-100&9.6&3.1&31.7 & 34.8 & 29.0 & \underline{43.0} & \textbf{67.1}
\\ 
  \cmidrule(lr){1-1} \cmidrule(lr){2-2} 
    \cmidrule(lr){3-10} 
 
\multirow{2}{*}{CIFAR10} &Clean&\textbf{97.3}&\underline{96.8}&65.2 & 53.5     & 52.4& 49.0 & 79.6 
\\ & PGD-100&8.1&2.5&  21.0 & 30.8   & 25.7& \underline{33.6} & \textbf{48.5}
\\ 
      \cmidrule(lr){1-1} \cmidrule(lr){2-2} 
    \cmidrule(lr){3-10} 
\noalign{\smallskip}
\multirow{2}{*}{CIFAR100} &Clean&\textbf{94.7}&\underline{92.1}&61.7 & 46.5  & 49.8& 50.5 & 64.1
\\ & PGD-100&2.7&0.0&18.3 & 26.1  & 18.6 & \underline{36.6} & \textbf{37.7}
\\ 
      
 
\specialrule{1.5pt}{\aboverulesep}{\belowrulesep}
 
\end{tabular}}
\end{subtable}
 
\end{table*}






==> Tables/Results.tex <==

\section{Experimental Results}


In this section, we perform extensive experiments to evaluate previous OOD detection methods, including the standard and adversarially trained ones, and our RODEO method against adversarial attacks. Our experiments are structured into three categories and are presented separately in sub-tables. The following subsections will provide an overview of each category.

 

 

 
\paragraph{ Novelty Detection :} 
 In this setup, for a dataset with $N$ classes, we conduct $N$ experiments and reported the average results across these experiments. In each experiment, we consider instances of a single class as in-distribution and all other instances as out-of-distribution. In our experiments, we conducted evaluations on both low-resolution and high-resolution datasets. By incorporating a mix of low-resolution and high-resolution datasets, our results provide insights into the generalizability and robustness of our method across different resolutions and domains. Table \ref{Table 1:Novelty Detection} provides the results of this setup, which indicates our superiority.

%We conduct several experiments in one-class classification, out-of-distribution detection, and open-set recognition. The evaluation metric that is used is the area under the receiver operating characteristics (AUROC), which provides a threshold-free measure of our method's performance. We evaluated our method against several attacks including BlackBox\cite{DBLP:journals/corr/abs-1905-07121}, PGD, and AutoAttack\cite{DBLP:journals/corr/abs-2003-01690}. All the attacks were performed with $\epsilon=\frac{8}{255}$ for low-resolution datasets and $\epsilon=\frac{2}{255}$ for high-resolution datasets. We also report our results where no adversarial attack is performed. To benchmark our method, we compared it against several existing methods in the respective domains. Significantly, RODEO exhibited substantial improvements over the majority of the compared methods, demonstrating its effectiveness and superiority.

% \textbf{One-Class classification}:
%  In this setup, for a dataset with $K$ classes, we conduct $K$ experiments and reported the average results across these experiments. In each experiment, we consider instances of a single class as in-distribution and all other instances as out-of-distribution. In experiments, we conducted evaluations on both low-resolution and high-resolution datasets. For the low-resolution datasets, we included CIFAR10\cite{krizhevsky2009learning}, CIFAR100\cite{krizhevsky2009learning}, MNIST\cite{lecun-mnisthandwrittendigit-2010}, and FashionMNIST\cite{xiao2017fashionmnist}. The results are available in Table \ref{Table 1.a:Novelty Detection for Low-Resolution}. Furthermore, we performed experiments on medical and industrial high-resolution datasets, namely Head-CT\cite{felipe-campos-kitamura_2018}, MVTec-ad\cite{bergmann2019mvtec}, Brain-MRI\cite{brainmri}, Covid19\cite{cohen2020covid}, and Tumor Detection\cite{msoud-nickparvar_2021} and reported the results in Table \ref{Table 1.b:Novelty Detection for High-Resolution}. By incorporating a mix of low-resolution and high-resolution datasets, our experiments provide insights into the generalizability and robustness of our method across different resolutions and domains.
\paragraph{Out-Of-Distribution Detection}
For the task of OOD detection, we considered CIFAR10 and CIFAR100 datasets as in-distribution datasets in separate experiments. Following earlier works\cite{chen2020robust}\cite{hendrycks2018deep}, we test the model over several out-of-distribution datasets which are disjoint from the in-distribution datasets, including MNIST, TinyImageNet\cite{imagenet}, Places365\cite{places}, LSUN\cite{LSUN}, iSUN\cite{iSUN}, Birds\cite{birds}, Flowers \cite{flowers}, COIL-100\cite{coil} and CIFAR10/CIFAR100 (depending on the in-ditribution dataset). The results are averaged over the mentioned datasets. We have brought the results of this task in Table \ref{Table2.a:OOD}.

\paragraph{Open-Set recognition:}
In this task, we divide each dataset into closed-set and open-set. The model is trained exclusively on samples from the closed set. The process was repeated five times, selecting a random set of classes as closed-set each time, and the average AUROC scores were reported. We conduct these experiments on CIFAR10, CIFAR100 labeled into 20 super-classes\cite{krizhevsky2009learning}, MNIST, and Fashion-MNIST which are used widely in the open-set literature. The number of classes present in closed-set is 
60\% of all classes. Table \ref{Table2.b:Open-Set Recognition} shows the superiority of RODEO in adversarial settings.


\paragraph{Baselines } 

\input{Tables/Results_Table}

==> Tables/Results_2.tex <==
% \begin{table*}[t]
%     \centering
%     \setlength{\tabcolsep}{4pt}
%     % Adjusting column spacing for compactness
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{ll*{5}{c}*{6}{c}c} 
%     % \toprule

%      \noalign{\smallskip}
%      \multirow{3}{*}{\textbf{\tenpt{Method}}}& \multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{\tenpt{Attack}}}} & \multicolumn{5}{c}{\textbf{\tenpt{Low-Res Datasets}}} &
%      \multicolumn{6}{c}{\textbf{\tenpt{High-Res Datasets}}} &
%      \multirow{3}{*}{\textbf{\tenpt{Mean}}}\\
%      \noalign{\smallskip}
%     \cmidrule(lr){3-7}  
%     \cmidrule(lr){8-13}  
%     & & \multirow{2}{*}{CIFAR10} & \multirow{2}{*}{CIFAR100} & \multirow{2}{*}{MNIST} & \multirow{2}{*}{FMNIST} & \multirow{2}{*}{SVHN} & \multirow{2}{*}{MVTecAD} & \multirow{2}{*}{Head-CT} & \multirow{2}{*}{BrainMRI} & \multirow{2}{*}{Tumor Detection} & \multirow{2}{*}{Covid19} & \multirow{2}{*}{Imagenet-30} \\ \\
%     \specialrule{0.8pt}{\aboverulesep}{\belowrulesep}
%     %& &  & \multirow{2}{*}{DeepSVDD} &  \multirow{2}{*}{MSAD} &  \multirow{2}{*}{Transformaly} &  \multirow{2}{*}{PatchCore} &  \multirow{2}{*}{PrincipaLS} &  \multirow{2}{*}{OCSDF} &  \multirow{2}{*}{APAE} &  \multirow{2}{*}{Ours*} &  \multirow{2}{*}{Ours} \\
%     %& & & & & & & & & & {\fontsize{5pt}{0pt}\selectfont(From-Scratch)} & {\fontsize{5pt}{0pt}\selectfont(Pre-Trained)} &  \\


%     \multirow{2}{*}{DeepSVDD} & 
    
%     Clean & & & & & & & & & & & & 1 \\
    
%     & PGD & & & & & & & & & & & & 1  \\
%     \specialrule{0.8pt}{\aboverulesep}{\belowrulesep}
    
%     \multirow{2}{*}{CSI} &
    
%     Clean & & & & & & & & & & & & 1  \\
    
%     &PGD & & & & & & & & & & & & 1  \\
%     \specialrule{0.8pt}{\aboverulesep}{\belowrulesep}
    
%     \multirow{2}{*}{MSAD} &
    
%     Clean & & & & & & & & & & & & 1  \\
    
%     &PGD & & & & & & & & & & & & 1  \\
    
%     \specialrule{0.8pt}{\aboverulesep}{\belowrulesep}
    
%     \multirow{2}{*}{Transformaly} &
    
%     Clean & & & & & & & & & & & & 1  \\
    
%     &PGD & & & & & & & & & & & & 1  \\
    
%     \specialrule{0.8pt}{\aboverulesep}{\belowrulesep}
    
%     \multirow{2}{*}{PatchCore} &
    
%     Clean & & & & & & & & & & & & 1  \\
%     &PGD & & & & & & & & & & & & 1  \\
    
%     \specialrule{0.8pt}{\aboverulesep}{\belowrulesep}
    
%     \multirow{2}{*}{PrincipaLS} &
    
%     Clean & & & & & & & & & & & & 1  \\
    
%     &PGD & & & & & & & & & & & & 1  \\
    
%     \specialrule{0.8pt}{\aboverulesep}{\belowrulesep}
%     \multirow{2}{*}{OCSDF} &
    
%     Clean & & & & & & & & & & & & 1  \\
    
%     &PGD & & & & & & & & & & & & 1 \\


%     \specialrule{0.8pt}{\aboverulesep}{\belowrulesep}
%     \multirow{2}{*}{APAE} &
    
%     Clean & & & & & & & & & & & & 1  \\
    
%     &PGD & 11 & 11 &11 &11 &11 &11 &11 &11 &11 &11 &11 &11.12 \\
    
%     \specialrule{0.8pt}{\aboverulesep}{\belowrulesep}  
    
%     \multirow{2}{*}{RODEO(ours)} &
    
%     Clean & & & & & & & & & & & & 1 \\
    
%     &PGD & & & & & & & & & & & & 1  \\

%     \multirow{2}{*}{RODEO(ours)} &
    
%     Clean & & & & & & & & & & & & 1 \\
    
%     &PGD & & & & & & & & & & & & 1  \\
    
%     \specialrule{0.8pt}{\aboverulesep}{\belowrulesep}
    
%     \end{tabular}}
%     % \caption{In the table presented, we evaluate the robustness of (One-Class) Novelty Detection methods across various datasets. Two adversarial attacks, namely PGD100 and AutoAttack, are considered, in addition to a clean setting without any adversarial attacks. For low-resolution datasets, a perturbation level of $ \epsilon = \frac{8}{255} $ was employed, while high-resolution datasets utilized $ \epsilon = \frac{2}{255} $. Results of our proposed method are distinctly reported in two configurations: from-scratch and pretrained. The most outstanding scores are highlighted in \textbf{bold}, with the second-best scores \underline{underlined}.}
%     \caption{In this table, we assess (One-Class) ND methods on various datasets against PGD100, AutoAttack (AA), and a clean setting, using the AUROC(\%) metric. Perturbations: $ \epsilon = \frac{8}{255} $ for low-res and $ \epsilon = \frac{2}{255} $ for high-res datasets. Our method's results are shown as from-scratch and pre-trained. Best scores are \textbf{bolded}; second-bests are \underline{underlined}.}


%     \label{Table1:Novelty Detection}
% \end{table*}


\begin{table}[ht]
% \setlength{\tabcolsep}{5pt}


\setlength{\tabcolsep}{8pt} % <-- Adjust this value to 
% increase/decrease the spacing between columns

\caption{In the table below, we assess OSR methods on datasets under PGD100 and clean setups, using AUROC(\%). Our results are reported in from-scratch and pre-trained.}
\vspace{0.1in} 
\resizebox{\columnwidth}{!}{
\begin{tabular}{ll*{5}{c}} 
\toprule
\noalign{\smallskip}



   % \multicolumn{1}{c}{Dataset} & \multicolumn{1}{c}{Attack}  &\multicolumn{6}{c}{Method }  
   %   \\      \cmidrule(lr){1-1} \cmidrule(lr){2-2} 
   %  \cmidrule(lr){3-9}  
    
    \multicolumn{1}{l}{\multirow{3}{*}{\textbf{\tenpt{Method}}}}& \multirow{3}{*}{\textbf{\tenpt{Attack}}} & \multicolumn{5}{c}{\textbf{\tenpt{Dataset}}} \\
    \cmidrule(lr){3-6}  
     & &\multirow{2}{*}{\textbf{MNIST}}&\multirow{2}{*}{\textbf{FMNIST}}&\multirow{2}{*}{\textbf{CIFAR10}} & \multirow{2}{*}{\textbf{CIFAR100}} 
   \\
 

\noalign{\smallskip\smallskip\smallskip}

\midrule



% capsnet: 1911.08616
% rest: ARAE 97.5	\_	64.1	73

\multirow{1}{*}{\textsc{ViT-MSP}} &Clean / PGD&\ul{92.4} / 2.9 & \ul{87.6} / 2.0 & \textbf{96.8} / 1.6 &\ul{92.1} / 0.0
\\ 
    %   \cmidrule(lr){1-1} \cmidrule(lr){2-2} 
    % \cmidrule(lr){3-10} 
\midrule

\multirow{1}{*}{$\text{\textsc{AT}}^*$} &Clean / PGD&80.2 / 36.1&72.5 / 29.8&65.2 / 20.6&61.7 / 17.9
%\\ & PGD&36.1&29.8&20.6&17.9
\\ 
\midrule
 
\multirow{1}{*}{\textsc{ATOM}} &Clean / PGD&74.8 / 4.1&64.3 / 4.2&68.3 / 5.0&51.4 / 2.6
%\\ & PGD&4.1&4.2&5.0&2.6
\\ 
\midrule

\noalign{\smallskip}
\multirow{1}{*}{\textsc{ALOE}} &Clean / PGD&79.5 / 37.3&72.6 / 28.5&52.4 / 25.6&49.8 / 18.2
%\\ & PGD&37.3&28.5&25.6&18.2
\\ 
\midrule
\noalign{\smallskip}

\multirow{1}{*}{\textsc{PLP}} &Clean / PGD& 88.3 / 0.4 & 82.6 / 0.0& \ul{94.1} / 0.0& \textbf{92.7} / 3.1
%\\ & PGD&  0.4& 0.0 &0.0  & 3.1
\\ 
\noalign{\smallskip}
\midrule

\multirow{1}{*}{\textsc{ATD}} &Clean / PGD&68.7 / \ul{56.5}&59.6 / \ul{42.1}&49.0 / \ul{32.4}&50.5 / \textbf{36.1}
%\\ & PGD&56.5&42.1&32.4&36.1
\\ 
\midrule
\noalign{\smallskip}
\multirow{2}{*}{\textsc{RODEO}} &Clean / PGD&\textbf{97.2} / \textbf{85.0}&\textbf{87.7} / \textbf{65.3}&79.6 / \textbf{62.7}&64.1 / \ul{35.3}
%\\ & PGD&85.0&65.3&62.7&35.3
\\ 
\noalign{\smallskip}
\cdashline{2-6}
\noalign{\smallskip}

& AA / A3 & 86.4 / 84.1& 66.8 / 62.9& 63.5 / 63.0& 36.9 / 35.4
%\\ & A3&84.1 &	62.9& 	63.0& 	35.4
\\ 
      
 
\bottomrule
 
\end{tabular}
}
\label{Table2.b:OSR}

\end{table}

\begin{table}[ht]
\setlength{\tabcolsep}{23pt} % <-- Adjust this value to increase/decrease the spacing between columns
\caption{In the table below, we assess OOD Detection techniques where CIFAR10 acts as the in-distribution and CIFAR100 as the out-of-distribution, along with the opposite configuration. This evaluation considers both the PGD100 attack and clean setups, with results based on the AUROC(\%). Perturbations are at $ \epsilon = \frac{8}{255} $. We showcase our method in from-scratch and pre-trained forms.  }
\vspace{0.1in} 
\resizebox{\columnwidth}{!}{
\begin{tabular}{ll*{3}{c}} 
\toprule
\noalign{\smallskip}


    \multicolumn{1}{l}{\multirow{3}{*}{\textbf{\tenpt{Method}}}}& \multirow{3}{*}{\textbf{\tenpt{Attack}}} & \multicolumn{2}{c}{\textbf{\tenpt{In-Dataset}}} \\
    \cmidrule(lr){3-4}  
     & &\multirow{2}{*}{\textbf{CIFAR10}}&\multirow{2}{*}{\textbf{CIFAR100}}
   \\
 

\noalign{\smallskip\smallskip\smallskip}

\midrule




\multirow{1}{*}{\textsc{ViT-MSP}} &Clean / PGD&\textbf{99.5} / 0.0&\textbf{95.1} / 0.0
%\\ & PGD&0.0&0.0
\\ 

\midrule

\multirow{1}{*}{$\text{\textsc{AT}}^*$} &Clean / PGD&80.5 / 18.9&70.0 / 12.7
%\\ & PGD&18.9&12.7
\\ 
\midrule
 
\multirow{1}{*}{\textsc{ATOM}} &Clean / PGD&82.7 / 24.4&91.6 / 3.6
%\\ & PGD&24.4&3.6
\\ 
\midrule

\noalign{\smallskip}
\multirow{1}{*}{\textsc{ALOE}} &Clean / PGD&97.8 / 5.0&79.3 / 24.9
%\\ & PGD&5.0&24.9
\\ 
\midrule
\noalign{\smallskip}

\multirow{1}{*}{\textsc{PLP}} &Clean / PGD& \ul{98.4} / 0.1 & \ul{93.7} / 0.0
%\\ & PGD& 0.1 &0.0 
\\ 
\midrule

\multirow{1}{*}{\textsc{ATD}} &Clean / PGD&94.3 / \ul{69.1}&87.7 / \ul{54.8}
%\\ & PGD&69.1&54.8
\\ 
\midrule
\noalign{\smallskip}
\multirow{2}{*}{\textsc{RODEO}} &Clean / PGD&93.2 / \textbf{69.5}&88.1 / \textbf{64.7}
%\\ & PGD&69.5&64.7
\\
\noalign{\smallskip}
\cdashline{2-4}
\noalign{\smallskip}
& AA / A3&69.0 / 68.8&65.3 / 63.2
%\\ & A3&68.8&63.2
\\ 
      
 
\bottomrule
 
\end{tabular}
}


\label{Table2.a:OOD}
\end{table}

% \caption{Out-of-distribution detection}
% \caption{In the table above, we assess OOD Detection methods using CIFAR10 vs. CIFAR100 evaluations and vice-versa, under the influence of the PGD100 attack and a clean setting. Perturbations were set at $ \epsilon = \frac{8}{255} $. Our method's results are presented in both from-scratch and pretrained configurations. Top scores are \textbf{bolded}, and the next best are \underline{underlined}.}    %   \cmidrule(lr){1-1} \cmidrule(lr){2-2}  
% capsnet: 1911.08616
% rest: ARAE 97.5	\_	64.1	73
    % \cmidrule(lr){3-10} 
    

==> Tables/Results_Table.tex <==
\begin{table*}[!htb]
\begin{subtable}{1\textwidth}
\caption*{Table 1: AUROC (\%) performance of ND methods on various datasets in a clean setting and under adversarial attacks using PGD100 and AutoAttack (AA). Perturbations for attacks are $\epsilon = \frac{8}{255}$ for low-resolution datasets and $\epsilon = \frac{2}{255}$ for high-resolution datasets. The best results are \textbf{bolded} and the second-best results are \underline{underlined}.}
% \resizebox{\linewidth}{!}{
\label{Table 1.a:Novelty Detection for Low-Resolutionn}
\begin{tabular}{lll*{13}{c}} 
\specialrule{1.5pt}{\aboverulesep}{\belowrulesep}
\noalign{\smallskip}


% The AUROC of various novelty detector models is utilized to evaluate their performance under different attacks. A clean evaluation is conducted on data that is not attacked, while other attacks refer to situations where both normal and abnormal data are attacked. 
  
   \multicolumn{2}{c}{\multirow{4}{*}{\Large{Dataset}}} & \multicolumn{1}{c}{\multirow{4}{*}{\Large{Attack}}} & &\multicolumn{7}{c}{Method }  
     \\      
    \cmidrule(lr){4-14}  

   
  & & &\multirow{2}{*}{DeepSVDD}&\multirow{2}{*}{CSI}&\multirow{2}{*}{MSAD} &\multirow{2}{*}{Transformaly}&\multirow{2}{*}{PatchCore} & \multirow{2}{*}{PrincipaLS} &\multirow{2}{*}{OCSDF} &\multirow{2}{*}{APAE}& RODEO    \\
  & & & & & & & & &  & & \small{(Ours)}  \\
  
\noalign{\smallskip}
 \specialrule{1.5pt}{\aboverulesep}{\belowrulesep}

\noalign{\smallskip}
% capsnet: 1911.08616
% rest: ARAE 97.5	\_	64.1	73
\multirow{8}{*}[-0.3cm]{\rotatebox[origin=c]{90}{\textbf{\Large{Low-Res}}}}
&

\multirow{2}{*}{CIFAR10} &Clean&64.8&94.3&\underline{97.2}&\textbf{98.3}&68.3&57.7&57.1&55.2&87.4
\\  &  &PGD / AA&23.4 / 9.7&2.8 / 0.0&0.0 / 0.0&0.0 / 0.0&0.3 / 0.0&\underline{24.1} / \underline{20.2}&22.0 / 15.3&0.1 / 0.0&\textbf{71.1}
 / \textbf{69.3}\\
 

      \cmidrule(lr){2-2} \cmidrule(lr){3-3} 
    \cmidrule(lr){3-14}   


\noalign{\smallskip}
% capsnet: 1911.08616
% rest: ARAE 97.5	\_	64.1	73
 
&\multirow{2}{*}{CIFAR100} &Clean&67.0&89.6&\underline{96.4}&\textbf{97.3}&66.8&52.0&48.2&51.8&79.6
\\&&PGD / AA&14.5 / 5.8&3.2 / 0.0&2.9 / 4.3&4.3 / 2.6&0.0 / 0.0&\underline{16.6} / \underline{14.7}&15.1 / 12.0&0.0 / 0.0&\textbf{62.8}
 / \textbf{61.0}\\
\cmidrule(lr){2-2} \cmidrule(lr){3-3} 
    \cmidrule(lr){3-14}   

\noalign{\smallskip}
% capsnet: 1911.08616
% rest: ARAE 97.5	\_	64.1	73
 
&\multirow{2}{*}{MNIST} & Clean&94.8&93.8&96.0&94.8&83.2&\underline{97.3}&95.5&92.5&\textbf{99.4}
\\&&PGD / AA&11.4 / 9.6&0.3 / 0.4&0.0 / 7.3&10.8 / 6.7&0.0 / 0.0&\underline{78.1} / \underline{72.5}&62.4 / 58.3&22.9 / 19.8&\textbf{95.7}
 / \textbf{95.2}\\
      \cmidrule(lr){2-2} \cmidrule(lr){3-3} 
    \cmidrule(lr){3-14}   




\noalign{\smallskip}
% capsnet: 1911.08616
% rest: ARAE 97.5	\_	64.1	73
 
&\multirow{2}{*}{Fashion-MNIST} &Clean& \underline{94.5}&92.7&94.2&94.4&77.4&91.0&90.6&86.1&\textbf{95.6}
\\&&PGD / AA&49.4 / 38.2&4.8 / 3.1&0.0 / 0.0&0.5 / 0.0&0.0 / 0.0&\underline{61.3} / \underline{58.2}
&54.5 / 49.2&11.2 / 7.0&\textbf{88.1}
 / \textbf{87.6}\\
      \cmidrule(lr){2-2} \cmidrule(lr){3-3} 
    \cmidrule(lr){3-14}   

 
\noalign{\smallskip}
% capsnet: 1911.08616
% rest: ARAE 97.5	\_	64.1	73
 
&\multirow{2}{*}{SVHN} &Clean& \underline{60.3}&96.0&63.1&55.4&52.1&63.0&58.1 &52.6&\textbf{78.6}
\\&&PGD / AA&7.7 / 2.8&1.3 / 0.4&0.6  / 2.5&7.6 / 5.8&3.2 / 0.1& \underline{31.4} / \underline{25.0}   &24.9 / 23.5&17.4 / 19.8&\textbf{45.4}
 / \textbf{41.2}\\
 
\specialrule{1.5pt}{\aboverulesep}{\belowrulesep}
\multirow{10}{*}[-0.3cm]{\rotatebox[origin=c]{90}{\textbf{\Large{High-Res}}}}
&\multirow{2}{*}{MVTecAD } &Clean&67.0&63.6&87.2&\underline{87.9}&\textbf{99.6}&63.8&58.7&62.1&61.5
\\&&PGD / AA&2.6 / 0.0&0.0 / 0.0&0.9 / 0.0&0.0 / 0.0&7.2 / 4.8&\textbf{24.3} / \underline{12.6}&5.2 / 0.3&4.7 / 1.8&\underline{15.9}
 / \textbf{14.2}\\

      \cmidrule(lr){2-2} \cmidrule(lr){3-3} 
    \cmidrule(lr){3-14}   


\noalign{\smallskip}
&\multirow{2}{*}{Head-CT} &Clean&62.5&60.9&59.4&78.1&\textbf{98.5}&68.9&62.4&68.1&\underline{87.3}
\\&&PGD / AA&0.0 / 0.0&0.6 / 0.0&0.0 / 0.0&6.4 / 3.2&1.5 / 0.0&\underline{27.8} / \underline{16.2}&13.1 / 8.5&6.6 / 3.8&\textbf{70.0}
 / \textbf{68.4}\\
       \cmidrule(lr){2-2} \cmidrule(lr){3-3} 
    \cmidrule(lr){3-14}    
  



\noalign{\smallskip}
% capsnet: 1911.08616
% rest: ARAE 97.5	\_	64.1	73
 
&\multirow{2}{*}{BrainMRI } & Clean&74.5&93.2&\textbf{99.9}&\underline{98.3}&91.4&70.2&63.2&55.4&76.3
\\&&PGD / AA&4.3 / 2.1&0.0 / 0.0&1.7 / 0.0&5.2 / 1.6&0.0 / 0.4&\underline{33.5} / \underline{17.8}&20.4 / 12.5&9.7 / 8.3&\textbf{71.1}
 / \textbf{70.5}\\

      \cmidrule(lr){2-2} \cmidrule(lr){3-3} 
    \cmidrule(lr){3-14}   


\noalign{\smallskip}
 
&\multirow{2}{*}{Tumor Detection} & Clean&70.8&85.3&\underline{95.1}&\textbf{97.4}&92.8&73.5&65.2&64.6&89.0
\\&&PGD / AA&1.7 / 0.0&0.0 / 2.2&0.1 / 0.0&7.4 / 5.1&9.3 / 6.1&\underline{25.2} / \underline{14.7}&17.9 / 10.1&15.8 / 8.3&\textbf{67.5}
 / \textbf{66.9}\\
  \cmidrule(lr){2-2} \cmidrule(lr){3-3} 
    \cmidrule(lr){3-14}   

\noalign{\smallskip}
% capsnet: 1911.08616
% rest: ARAE 97.5	\_	64.1	73
 
&\multirow{2}{*}{Covid19} & Clean&61.9&65.1&89.2&\textbf{91.0}&77.7&54.2&46.1&50.7&\underline{79.6}
\\&&PGD / AA&0.0 / 0.0&0.0 / 0.3&4.7 / 1.9&10.6 / 4.4&4.2 / 0.5&\underline{15.3} / \underline{9.1}&9.0 / 6.5&11.2 / 8.7&\textbf{59.4}
 / \textbf{58.8}\\
 \cmidrule(lr){1-14} 
 &\multirow{2}{*}{\textbf{Mean}} & Clean& 71.8& 83.4& \underline{87.8}& \textbf{89.3}& 80.8& 69.2& 64.5& 63.9& 83.4
\\&&PGD / AA & 11.5 / 6.8& 1.3 / 0.6& 1.1 / 1.6& 5.3 / 2.9& 2.6 / 1.2& \underline{33.8} / \underline{26.1}& 24.4 / 19.6& 10.0 / 7.7& \textbf{64.7} / \textbf{63.3}\\
\specialrule{1.5pt}{\aboverulesep}{\belowrulesep}
\end{tabular}
% }

\end{subtable}
    \begin{subtable}{1\textwidth}
    \begin{minipage}[t*]{.49\linewidth}
    \caption*{Table 2: AUROC (\%) performance of OOD detection methods, where CIFAR-10 and CIFAR-100 are considered as separate inlier datasets in each experiment. The union of other datasets are used as OOD data. This evaluation considers both the PGD-100 attacked and clean setups. Perturbations for attacks are $\epsilon = \frac{8}{255}$.}
    \label{Table2:a:OOD}
\resizebox{\linewidth}{!}{
\begin{tabular}{ll*{9}{c}} 
\specialrule{1.5pt}{\aboverulesep}{\belowrulesep}
\noalign{\smallskip}

   \multirow{3}{*}{\large{In-Dataset}} & \multirow{3}{*}{\large{Attack}}  &\multicolumn{8}{c}{Method}\\
    \cmidrule(lr){3-10}  
    
  &&\multirow{1}{*}{ViT-MSP}&AT$^{*}$ & \multirow{1}{*}{ATOM} & \multirow{1}{*}{ALOE}& \multirow{1}{*}{ATD} &  RODEO& 
 \\
\noalign{\smallskip}
 \hline
\noalign{\smallskip}
% capsnet: 1911.08616
% rest: ARAE 97.5	\_	64.1	73
 
\multirow{2}{*}{CIFAR10}
&\multirow{1}{*}{\centering Clean}&\textbf{99.5}&80.5&82.7&\ul{97.8}&94.3 & 93.2 \\&\multirow{1}{*}{\centering PGD}&0.0&20.8&25.1&6.0&\underline{69.3}& \textbf{70.4}\\

\noalign{\smallskip}
 \hline
\noalign{\smallskip}
 
\multirow{2}{*}{CIFAR100}
&\centering Clean&\textbf{95.1}& 70.0&\ul{91.6}&79.3&87.7& 88.1& \\
&\centering PGD&0.0&13.6&5.4&26.4&\underline{55.3}& \textbf{66.4}  \\
\specialrule{1.5pt}{\aboverulesep}{\belowrulesep}
    \end{tabular}}
\scriptsize{* AT indicates the model was trained without using OE.}
    \end{minipage}%
    \hspace{\fill}
    \begin{minipage}[t*]{.49\linewidth}
    \flushright
    \caption*{Table 3: AUROC (\%) performance of OSR methods on various datasets in a clean setting and under PGD-100 attack.\label{Table2.b:Open-Set Recognition}}
        \resizebox{\linewidth}{!}{\begin{tabular}{ll*{9}{c}} 
 \specialrule{1.5pt}{\aboverulesep}{\belowrulesep}
 \noalign{\smallskip}



   \multirow{3}{*}{\large{Dataset}} & \multirow{3}{*}{\large{Attack}}  &\multicolumn{6}{c}{Method }  
     \\   
    \cmidrule(lr){3-9}  


  &&\multirow{1}{*}{ViT-MSP}&AT$^{*}$ & \multirow{1}{*}{ATOM} & \multirow{1}{*}{ALOE}& \multirow{1}{*}{ATD} &  RODEO  &   
 \\
 
\noalign{\smallskip}
 \hline
\noalign{\smallskip}



% capsnet: 1911.08616
% rest: ARAE 97.5	\_	64.1	73

\multirow{2}{*}{MNIST} &Clean&\ul{92.4}&80.2 & 74.8   & 79.5& 68.7 &\textbf{97.2}
\\ & PGD&4.2&36.2 & 6.3 & 38.2& \underline{56.7} & \textbf{88.8}
\\ 
      \cmidrule(lr){1-1} \cmidrule(lr){2-2} 
    \cmidrule(lr){3-10} 


\multirow{2}{*}{FMNIST} &Clean&\underline{87.6}&72.5 & 64.3  & 72.6& 59.6 & \textbf{87.7}
\\ & PGD&3.1&31.7 & 4.7 & 29.0 & \underline{43.0} & \textbf{67.1}
\\ 
  \cmidrule(lr){1-1} \cmidrule(lr){2-2} 
    \cmidrule(lr){3-10} 
 
\multirow{2}{*}{CIFAR10} &Clean&\textbf{96.8}&65.2 & 68.3 & 52.4& 49.0 & \ul{79.6} 
\\ & PGD& 2.5& 21.0 & 5.2 & 25.7& \underline{33.6} & \textbf{48.5}
\\ 
      \cmidrule(lr){1-1} \cmidrule(lr){2-2} 
    \cmidrule(lr){3-10} 
\noalign{\smallskip}
\multirow{2}{*}{CIFAR100} &Clean&\textbf{92.1}&61.7 & 51.4  & 49.8& 50.5 & \ul{64.1}
\\ & PGD&0.0&18.3 & 3.2  & 18.6 & \underline{36.6} & \textbf{37.7}
\\ 
\specialrule{1.5pt}{\aboverulesep}{\belowrulesep}
\end{tabular}}
\raggedright
\scriptsize{* AT indicates the model was trained without using OE.}
 \end{minipage} 
    \end{subtable}
\end{table*}

==> Tables/Seperate_FDC.tex <==
\begin{subtable}{1\textwidth}
\centering
\caption*{Table 5: Comparison of generated outliers by different OE techniques using the $FDC$ metric. A higher value indicates that the generated outliers have more diversity and are closer to the corresponding normal dataset (target dataset). The experiments were conducted in the ND setting.\label{Table:Ablation_1}}
%\caption{FDC metric for different exposure techniques.}\label{Table:Ablation_12}
\setlength{\tabcolsep}{12pt} % Adjusting column spacing for compactness
\resizebox{\linewidth}{!}{
\begin{tabular}{l*{14}{c}}
\specialrule{1.5pt}{\aboverulesep}{\belowrulesep}
\multicolumn{1}{c}{\multirow{2}{*}{\large{Exposure Technique}}} &\multicolumn{6}{c}{\large{Target Dataset}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\large{Mean}}}} \\
\cmidrule{2-7}
& \small{CIFAR10}&\small{MNIST}&\small{FMNIST}&\small{MVTec-ad}&\small{Head-CT}& \small{Covid19}&  \\
\specialrule{1.5pt}{\aboverulesep}{\belowrulesep}

\multirow{1}{*}{Gaussian Noise} & 0.822 & 0.704 & 0.810 & 0.793 & 0.735 & 0.674 & 0.756 \\

\cmidrule(lr){1-1}
\cmidrule(lr){2-11}
\cmidrule(lr){12-12}

\multirow{1}{*}{Vanilla OE (ImageNet)} & \underline{7.647} & 0.795 & \underline{2.444} & 1.858 & \underline{3.120} & \underline{3.906} & \underline{3.295} \\


 \cmidrule(lr){1-1}
\cmidrule(lr){2-11}
\cmidrule(lr){12-12}

\multirow{1}{*}{Mixup with ImageNet} & 2.185 & 0.577 & 0.985 & 1.866 & 1.587 & 2.078 & 1.547 \\


\cmidrule(lr){1-1}
\cmidrule(lr){2-11}
\cmidrule(lr){12-12}

\multirow{1}{*}{Fake Image Generation} & 0.987 & 0.649 & 0.907 & 1.562 & 0.881 & 0.896 & 0.980 \\

\cmidrule(lr){1-1}
\cmidrule(lr){2-11}
\cmidrule(lr){12-12}


\multirow{1}{*}{Stable Diffusion Prompt} & 1.359 & \underline{1.790} & 1.399 & \textbf{1.982} & 1.097 & 0.654 & 1.381 \\



\cmidrule(lr){1-1}
\cmidrule(lr){2-11}
\cmidrule(lr){12-12}

\multirow{1}{*}{\textbf{Adaptive OE (Ours)}} & \textbf{8.504} & \textbf{11.395} & \textbf{3.819} & \underline{1.948} & \textbf{12.016} & \textbf{5.965} & \textbf{6.687} \\
\specialrule{1.5pt}{\aboverulesep}{\belowrulesep}

\end{tabular}
}
\end{subtable}

==> Tables/Unlabeled_OSR_OOD.tex <==
% \begin{table}
% \centering
% \begin{tabular}{| *{8}{c|} }
% \hline

% \hline

% dataset & \tiny {RODEO,4/255,(pretrain)}  & \tiny {RODEO,8/255,(pretrain)} &\tiny {RODEO,4/255,( scratch) }&\tiny { RODEO,eps=8/255,( scratch)}& \tiny {ATD 4/255 }& \tiny {ATD 8/255} \\

% \hline
% Cifar10 & 76.23 - 50 & 76.22 - 36.25 & 72.16 - 46.49 & 65.76 - 31.25 & 57.41 - 43.74 & 48.94 - 33.63\\
% \hline
% Cifar100 & & 65.21 - 27.53 & 66.69 - 49.13 & 62.60 - 39.93 & & \\
% \hline
% Mnist & 97.04 - 95.15 & 97.57 - 94.91 & 97.73 - 94.76 & 95.97 - 87.15 & & \\
% \hline
% FashionMnist& 78.60 - 66.70 & 84.39 - 66.92 & 76.80 - 61.34 & 71.90 - 53.58 & & \\
% \hline
% SVHN & & & 72.45 - 31.94 & 71.22 - 14.22 & & \\
 
% \hline
% \end{tabular}
% \caption{OSR}
% \label{tab:example}
% \end{table}


%


% \begin{table}
% \centering
% \begin{tabular}{|c|c|c|c|c| }
% \hline
% Column 1 & Column 2 & Column 3 & Column 4 & Column 5   \\


% datasets&\tiny {RODEO,8/255,(pretrain)} & \tiny {RODEO,4/255,(pretrain)}&\tiny {RODEO,4/255,( scratch) }&\tiny { RODEO,eps=8/255,( scratch)}  \\

% \hline
% Cifar10 & 92 - 72.3 & 95.1 - 83.09 & & 87.3 - 70  \\
% \hline
% Cifar100 & 88.7 - 68.5 & 92.73 - 77.87 & 84.2 - 72.225 & 79.555 - 64.755 \\
% \hline
% Mnist & & & &   \\
% \hline
% FashionMnist& & & &   \\
% \hline
% SVHN & 80.9 - 29.63 & & &   \\
 


% line
% \end{tabular}
% \caption{ND (One Class )}
% \subcaption*{(a) Comparison of AUROC of SOTA to our proposed method in the regular ND setting. }

% \label{tab:example}
% \end{table}


% \begin{table}[h!]
%   \centering
%   \begin{tabular}{ |c|c|c|c|c|c|c| }
%   \hline
%     & ALOE (MSP / ODIN) & Clip AD(From Scratch Version) & ATD(Clean/Roubst) & OE (Hendryks) & OE (Ruff) & PANDA(Clean/Roubst) \\
%   \hline
%   MNIST & 3.17 / 4.05 & 56.87 & 47.29/4.21 &  &  & 89.37/0.00  \\
%   \hline
%   SVHN & 3.22 / 3.90 & 64.54 & 78.64/33.86 &  &  & 89.75/0.00  \\
%   \hline
%   Imagenet-30 & 24.70 / 23.31 & 77.50 & 83.08/37.43 &  &  & 98.04/0.00 \\
%   \hline
%   Gaussian & 1.27 / 3.10 & 57.06 & 52.08/2.37  &  &  &  85.47/0.00  \\
%   \hline
%   Row 5 &  &  &  &  &  &  \\
%   \hline
%   Row 6 &  &  &  &  &  &  \\
%   \hline
%   Row 7 &  &  &  &  &  &  \\
%   \hline
%   Row 8 &  &  &  &  &  &  \\
%   \hline
%   Row 9 &  &  &  &  &  &  \\
%   \hline
%   Row 10 &  &  &  &  &  &  \\
%   \hline
%   \end{tabular}
%   \centering
%   \caption{Outlier Comparison - IN:CIFAR10 , OUT:CIFAR100}
% \end{table}









 








%\begin{table*}[h ]
 
% \centering
% \caption{ Table1: Unlabeled multi class
% }\label{Table:Main_Results}
% \subcaption*{Table1-a }
% \resizebox{\linewidth}{!}{\begin{tabular}{llr*{13}{c}} 
% \hline\noalign{\smallskip}



%    \multicolumn{1}{c}{Dataset} & \multicolumn{1}{c}{Attack} & &\multicolumn{7}{c}{Method }  
%      \\      \cmidrule(lr){1-1} \cmidrule(lr){2-2} 
%     \cmidrule(lr){3-13}  
   
%   & &DeepSVDD&CSI&MSAD &Transformaly&PatchCore & PrincipaLS & RFFAD& OCSDF &SOAP& RODEO  & RODEO+    \\
% \noalign{\smallskip}
%  \hline
% \noalign{\smallskip}
% % capsnet: 1911.08616
% % rest: ARAE 97.5	\_	64.1	73
 
% \multirow{2}{*}{CIFAR10} &Clean&x&x&x & 1& 2 & 0 & 1& 2 & 2 & 2& 2
% \\ & PGD-10&x&x&x & 1& 2 & 0 & 1& 2 & 2 & 2& 2
% \\ 
%       \cmidrule(lr){1-1} \cmidrule(lr){2-2} 
%     \cmidrule(lr){3-13} 


% \multirow{2}{*}{CIFAR100} &Clean&x&x&x & 1& 2 & 0 & 1& 2 & 2 & 2& 2
% \\ & PGD-10&x&x&x & 1& 2 & 0 & 1& 2 & 2 & 2& 2
% \\ 
%       \cmidrule(lr){1-1} \cmidrule(lr){2-2} 
%     \cmidrule(lr){3-13} 

% \multirow{2}{*}{MNIST} &Clean&x&x&x & 1& 2 & 0 & 1& 2 & 2 & 2& 2
% \\ & PGD-10&x&x&x & 1& 2 & 0 & 1& 2 & 2 & 2& 2
% \\ 
%       \cmidrule(lr){1-1} \cmidrule(lr){2-2} 
%     \cmidrule(lr){3-13} 


% \multirow{2}{*}{Fashion-MNIST} &Clean&x&x&x & 1& 2 & 0 & 1& 2 & 2 & 2& 2
% \\ & PGD-10&x&x&x & 1& 2 & 0 & 1& 2 & 2 & 2& 2
% \\ 
  
 
% \hline
 
% \end{tabular}}
% \end{table*}
 


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

